Data-Efficient Contrastive Language-Image Pretraining: Prioritizing Data Quality over Quantity

Contrastive Language-Image Pre-training (CLIP) on large-scale image-caption datasets learns representations that can achieve remarkable zero-shot generalization. However, such models require a massive amount of pre-training data. Improving the quality of the pre-training data has been shown to be much more effective in improving CLIP's performance than increasing its volume. Nevertheless, finding small subsets of training data that provably generalize the best has remained an open question. In this work, we propose the first theoretically rigorous data selection method for CLIP. We show that subsets that closely preserve the cross-covariance of the images and captions of the full data provably achieve a superior generalization performance. Our extensive experiments on ConceptualCaptions3M and ConceptualCaptions12M demonstrate that subsets found by \method\ achieve over 2.7x and 1.4x the accuracy of the next best baseline on ImageNet and its shifted versions. Moreover, we show that our subsets obtain 1.5x the average accuracy across 11 downstream datasets, of the next best baseline. The code is available at: https://github.com/BigML-CS-UCLA/clipcov-data-efficient-clip.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> notation.tex <==

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}

==> old_versions/v0_method.tex <==
\section{Multimodal Subsets that Generalize on Par with the Full Data}\label{sec:method}
We start by investigating which properties the subset $S$ must satisfy, such that the learned representations on the subset provide a similar downstream linear probe and zero-shot classification error to that of the full data.

\subsection{Background}
Consider the joint data distribution $\pmm(x_v, x_l)$, where $\pmm \in \mathbb{R}^{N_V \times N_L}$ can be formulated a co-occurrence matrix between all visual-language data pairs \citep{pmlr-v202-zhang23an}: 
% such that $\pmm(x_v, x_l)\geq 0, \forall x_v \in [N_V], x_l \in [N_L]$.
%
% As in \cite{pmlr-v202-zhang23an}, we start by formulating the joint distribution $\pmm(x_v, x_l)$ as a co-occurrence matrix $A \in \mathbb{R}^{N_V \times N_L}$ between all images and captions, where 
\begin{equation}
A(x_v, x_l) = \pmm(x_v, x_l) \geq 0, \forall \xv \in \Xv, \forall \xl \in \Xl.
\end{equation}
%%
Contrastive multimodal learning with spectral loss defined in Eq. \ref{eq:spectral} is equivalent to the asymmetric matrix factorization for the normalized co-occurrence matrix
$\tilde{A}$ 
\begin{equation}
L_{AMF}(\tilde{F_V}, \tilde{F_L}) := \norm{\tilde{A} - \tilde{F_V} \tilde{ F_L}^\top}^2,
\end{equation}
where ${F_V} \in \mathbb{R}^{N_V \times q}, {F_L} \in \mathbb{R}^{N_L \times q}$ are matrices containing the image and text representations, computed using the vision and language encoders $f_V, f_L$, and $\tilde{A}$ is the co-occurence matrix %obtained by performing two-sided normalization 
$\tilde{A}_{\xv, \xl} := \frac{A_{\xv, \xl}}{\sqrt{\pv(\xv) \pl(xl)}}$, normalized by marginal probabilities of image $x_v$, i.e., $\pv(\xv) := \sum_\xv A_{\xv, \xl}$, and text $x_l$, i.e., $\pl(\xl) := \sum_\xl A_{\xv, \xl}$.
% \textbf{\sj{Linear Probe Error}}
% \begin{theorem}[\sj{modified version of Lemma B.1 from \cite{zhang2023generalization}}]\label{thm:lp_error}
% Let $(f_V^*, f_L^*)$ be a minimizer of the population loss $L_{SCL}(f_V, f_L)$

Then, the linear probe error $\errlp{f_V^*}$ for a downstream taks with labels $y$ is upper-bounded by:
\begin{equation}
\errlp{f_V^*} \leq \frac{2\phi^y}{1 - \sigma^2_{k+1}} + 8\alpha_y.
\end{equation}
% \end{theorem}
The linear probe error depends on $\sigma_{k+1}$, conductance $\phi$, and labeling error $\alpha$, defined below.

\textbf{Singular values of $\pmb{\tilde{A}}$} $\sigma_1 \geq \cdots \geq \sigma_q$ are singular values of $\tilde{A}$, 
%$\pmb{\sigma_{k+1}}$ is the $k+1^{th}$ largest singular value of $\tilde{A}$ 
capturing the connectivity of the specified by $A$. Larger singular value of $\tilde{A}$ correspond to better connectivity. 
% and $\phi$ and $\alpha$ are defined as follows:

\textbf{Conductance ($\pmb{\phi}$)} captures the probability of image and text from different classes to co-occur:
\begin{align}
    \phi^y &= \sum_{\xv, xl} \pmm(\xv, \xl) \mathbbm{1}[y(\xv) \neq y(\xl)].
    % \alpha_y &= \E_{\xv, \xl} \mathbbm{1}[{y}(\xv)\neq y(\xl)].
\end{align}
%%%
\textbf{Labeling error $\pmb{\alpha}$} is labeling error capturing discrepancy in labels between the image-caption pairs:
\begin{align}
    % \phi^y &= \sum_{\xv, xl} \pmm(\xv, \xl) \mathbbm{1}[y(\xv) \neq y(\xl)],\\
    \alpha_y &= \E_{\xv, \xl} \mathbbm{1}[{y}(\xv)\neq y(\xl)].
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Let $y$ be the labeling function associated with a given downstream task s.t. $y(x) := i$ if $x$ belongs to latent class $i$. 

% \begin{definition}[Labeling Error for Task Specified by $y$]
% \begin{equation}
%     \alpha_y = \E_{\xv, \xl} \mathbbm{1}[{y}(\xv)\neq y(\xl)],
% \end{equation}
% \end{definition}

% \begin{definition}[Conductance for Task Specified by $y$]
%     \begin{equation}
%         \phi^y = \sum_{\xv, xl} \pmm(\xv, \xl) \mathbbm{1}[y(\xv) \neq y(\xl)]
%     \end{equation}
% \end{definition}


% \begin{theorem}[ZS error]\label{thm:zs_error}

% $\tilde{F_V}$ are the \sj{normalized?} image and caption representation matrices, respectively i.e. the $\xv$-th row of $\tilde{F_V} = \pv(\xv) \fv{\xv}$ and the $\xl$-th row of $\tilde{F_L} = \pl(\xl) \fl{\xl}$.

% Furthermore, define ${F_V} \in \mathbb{R}^{N_V \times k}$ as the matrix containing the representations of the images, computed using vision encoder $f_V$, i.e. the $\xv$-th row of ${F_V}$ is exactly $\fv{\xv}$. Similarly,  let ${F_L} \in \mathbb{R}^{N_L \times k}$ be the matrix containing the representations of the images, computed using vision encoder $f_L$, i.e. the $\xv$-th row of ${F_L}$ is exactly $\fv{\xl}$. 


% \cite{pmlr-v202-zhang23an} showed that low-rank matrix factorization objective on the normalized co-occurence matrix $\tilde{A}$ $$L_{AMF}(\tilde{F_V}, \tilde{F_L}) := \norm{\tilde{A} - \tilde{F_V} \tilde{ F_L}^\top}^2_F$$ where $\tilde{F_V}$ are the \sj{normalized?} image and caption representation matrices, respectively i.e. the $\xv$-th row of $\tilde{F_V} = \pv(\xv) \fv{\xv}$ and the $\xl$-th row of $\tilde{F_L} = \pl(\xl) \fl{\xl}$. 


\begin{comment}
\textbf{\sj{MMCL = AMF}}
\begin{theorem}[Theorem 3.1 from \cite{pmlr-v202-zhang23an}]\label{thm:mmcl=amf}
\sj{drop?: Let the $\xv$-row of $F_V$ and the
$\xl$-row of $F_L$ represent the corresponding encoded features of these samples in the following form, ${(F_V)}_\xv = \sqrt{\pv_(\xv)} \fv{\xv}^\top$ and ${(F_L)}_\xl = \sqrt{\pl (\xl)} \fl{\xl}^\top$}

Then the low-rank asymmetric matrix factorization loss is equivalent to the multi-modal contrastive loss up to a constant,
$$L_{AMF}(F_V, F_L) = L_{SCL}(f_V, f_L) + const.$$
\end{theorem}

Using this equivalence, \cite{pmlr-v202-zhang23an} proves that the generalization error of multi-modal contrastive learning on a given downstream task can be determined by the labeling error , the conductance and the k+1-th largest singular value of the normalized co-occurrence matrix.

In particular, the downstream generalization errors using linear probe and zeroshot classification can be bound as follows:

% \end{theorem}

\textbf{Labeling error} $\alpha_y$ accounts for the discrepancy in labels between the image-caption pairs, which can vary in practice based on how the dataset is generated.

\textbf{Singular Value} According to the spectral graph theory \citep{chung_1997}, the singular values  represent the connectivity of the bipartite graph specified by $A$. Larger singular value of $\tilde{A}$ correspond to better connectivity. 
\end{comment}


\subsection{Finding Generalizable Multimodal Subsets}
We rely on the above observations to find subsets $S \subset V$ of size $|S|\leq k$ that provide very similar generalization performance to that of the full data, on various downstream tasks. Such subsets should (1) best preserve the singular values $\sigma_i$ of the normalized co-occurrence matrix $\tilde{A}$, (2) have a small conductance $\phi$, and (3) small labeling error $\alpha$. Ensuring (1), (2) and (3) pn the subset $S$, given that every example in $V \setminus S$ is sufficiently similar to the examples in $S$, guarantees good generalization on the entire population. 
% \sj{del?: In addition, to ensure a superior generalization performance on the entire population we also require that (4) the selected subset to be similar to all the examples in $V$.}

Let $M_{R, C}$ be the matrix where $\forall r \in R, \forall c \in C, M_{r, c} = 1$ and 0 everywhere else. 

\begin{lemma}[MMCL on Subset is AMF on Masked $\tilde{A}$]\label{lemma:subset_mmcl}
$\exists$ constant $c$ s.t.

$$c^2 L_{SCL}^S(f_V, f_L) + const. = \norm{M_{S, S} \odot \tilde{A} - F_V F_L^\top}^2$$

\end{lemma}

Proof in Appendix \ref{app:proof:lemma:subset_mmcl}. 

% Since, the generalization performance of multi-modal contrastive learning can be determined by the conductance, the singular value of $\tilde{A}$ and labeling error, a subset that preserves the conductance, connectivity and labeling error of the full data achieves similar generalization performance to the full data. 

\paragraph{Preserving the Spectrum of the Normalized Co-occurrence Matrix}

We start by finding subsets that best preserve the spectrum of the normalized co-occurrence matrix $\tilde{A}$. As shown in Lemma \ref{lemma:subset_mmcl}, training on the subset $S\subset V$ can be modeled as learning representations that recover the masked normalized co-occurrence matrix $M_{S, S} \odot \tilde{A}$. 

%This ensures that the generalization guarantees on the subset extend to the true population. 

%Let $\At_S$ the matrix that captures the masked normalized co-occurrence matrix and the similarities i.e. $$\At_S = M_{S, S} \odot \tilde{A} + \underbrace{M_{S, V \setminus S} \odot \At}_{\text{sim. between image in $S$ and caption in $V \setminus S$}} +  \underbrace{M_{V \setminus S, S} \odot \At}_{\text{sim. between caption in $S$ and image in $V \setminus S$}}$$

Selecting a subset $S\subset V$ can be modeled as perturbing the normalized co-occurrence matrix $\tilde{A}$, where the norm of the perturbation  $\norm{E}=\norm{\tilde{A}-M_S\odot \tilde{A}}$, is a function of the sum of entries in $\tilde{A}$ that are zeroed out. Therefore, the subset that minimizes the upper-bound of change on the singular values of $\tilde{A}$ is the one that has the smallest norm of error $\|E\|$, g

%Formally, we wish to solve:
 %\begin{equation}
  %   S^*_{\sigma}\in \argmin \|\tilde{A}-M_S\odot \tilde{A}\|. \quad 
 %\end{equation}

%To bound the error in preserving the spectrum, we rely on Weyl’s theorem \citep{weyl1912asymptotic}
%stating that under bounded perturbations $E$ to a matrix, no singular value can move more than the norm of the perturbations. Formally, $|\sigma'_i - \sigma_i|\leq \norm{E}$, where $\sigma'_i$ and $\sigma_i$ are the singular values of the $M_{S, S} \odot \At$ and original normalized co-occurrence matrix respectively.

%Therefore, the subset that minimizes the upper-bound of change on the singular values of $\tilde{A}$ is the one that has the smallest norm of error $\|E\|$. %Formally, we wish to solve:
%Selecting a subset $S\subset V$ can be modeled as perturbing the normalized co-occurrence matrix $\tilde{A}$, where the norm of the perturbation  $\norm{E}=\norm{\tilde{A}-M_S\odot \tilde{A}}$, is a function of the sum of entries in $\tilde{A}$ that are zeroed out. Therefore, the subset that minimizes the upper-bound of change on the singular values of $\tilde{A}$ is the one that has the smallest norm of error $\|E\|$. %Formally, we wish to solve:
% \begin{equation}
%     S^*_{\sigma}\in \argmin \|\tilde{A}-M_S\odot \tilde{A}\|.
% \end{equation}

\begin{lemma}\label{lemma:errsv_bound}[singular value error]
For any subset $S \subseteq V$, the error on the singular values of the normalized co-occurrence matrix is upper-bounded as follows: 

\end{lemma}
The proof can be found in Appendix \ref{app:proof:lemma:errsv_bound}.

\begin{align}
\errsv = {|\sigma_r - \sigma_r^S|}^2 \leq \norm{A}^2 - \frac{1}{2} \sum_{y} \Big [ &\sum_{i,j \in S_y} {\At(x_v^i,x_l^j)}^2 + {\At(x_v^j,x_l^i)}^2 \nonumber\\
& + \sum_{i \in S_y} \sum_{j \in S_{y'\neq y}} {\At(x_v^i,x_l^j)}^2 + {\At(x_v^j,x_l^i)}^2 \Big ] % r\in[q]   
\end{align}


% deleted old eq
\iffalse
\begin{equation}
\errsv = {|\sigma_r - \sigma_r^S|}^2 \leq \norm{A} - \sqrt{\frac{1}{2} \sum_{i \in S} \sum_{j \in S} {\At(x_v^i,x_l^j)}^2 + {\At(x_v^j,x_l^i)}^2}  \quad \forall r\in[q]   
\end{equation}
\fi

% deleted section on intra-class connectivity
\iffalse
\textbf{Ensuring sufficient intra-class connectivity between $S$ and $V \setminus S$}

To guarantee good generalization on the true population, we need the vision and language encoders trained on the subset to preserves the similarities between the representations of $S$ and $V \setminus S$ in every latent class. 
Let $\errcc$ be defined as the intra-class connectivity between $S$ and $V$ i.e. $\errc = \frac{1}{2} \sum_{i \in S_y}\sum_{j \in V_y \setminus S_y}  {\At(x_v^i,x_l^j)}^2 + {\At(x_v^j,x_l^i)}^2$
\fi

The subset that (1) best preserve the singular values $\sigma_i$ of the normalized co-occurrence matrix  $\At$, (2) have a small conductance $\phi$, and (3) small labeling error $\alpha$ can be found by maximizing the objectives in Eq. \ref{obj:sigma}, \ref{obj:phi}, \ref{obj:alpha}: 
\begin{equation}
    S^*\in\argmax_{S\subset V, |S|\leq k} F_{\sigma}(S)+F_{\phi}(S)+2F_{\alpha}(S).
\end{equation}

We see that the subset that minimizes the error on the singular values can be found as well as the  maximizing the following non-monotone submodular\footnote{A set function $F : 2^V \rightarrow \mathbb{R}^+$ is submodular if $F(e|S) = F(S \cup \{e\})-F(S) \geq F(T \cup \{e\})-F(T)$, for any $S \subseteq T \subseteq V$ and $e \in V \setminus T$. $F$ is monotone if $F(e|S) \geq 0$ for any $e \in V \setminus S$
and $S \subseteq V$.} function:
\begin{equation}\label{obj:sigma}
    % S^*_{\sigma}\in \argmax_{S \subseteq V, |S|\leq k} 
    F_{\sigma}(S) = \sum_{i \in S} \sum_{j\in S} {\At(x_v^i,x_l^j)}^2 + {\At(x_v^j,x_l^i)}^2.
\end{equation}
The subset that maximizes the above objective covers the largest entries of $\At$.

\paragraph{Achieving Small Conductance}
To find subsets with small conductance, we need to minimize the connectivity between images and text in different classes.

\begin{lemma}\label{lemma:errc_bound}[conductance error]
For any subset $S \subseteq V$, and a given labeling $y$, the difference between the 
conductance of the subset $\phi_S^y$ and full data is upper-bounded as follows: 
% \begin{equation}
%     % \errc = \phi^y - \phi^y_S
%     % \leq \phi^y -
%     F_{\phi}(S)=\phi_S^y= \sum_{\substack{\xv \in \Xv^S \\ \xl \in \Xl^S}} \mathbbm{1}[y(\xv) \neq y(\xl)] A(\xv,\xl).
% \end{equation}

% Note that $S \subset \Xv^S \times \Xl^S$

% old 15, which is not the definition, so this is not an equality: 
% \begin{equation}
%     % \errc = \phi^y - \phi^y_S
%     % \leq \phi^y -
%     F_{\phi}(S)=\phi_S^y= \sum_{\substack{(\xv, \xl) \in S}} \mathbbm{1}[y(\xv) \neq y(\xl)] A(\xv,\xl).
% \end{equation}
\begin{equation}
        \errc = \phi_S^y -\phi^y \leq \sum_y \sum_{i\in S_y} \sum_{j\in S_{y'\neq y}} \Big[ A(x_v^i,x_l^j)+A(x_v^j,x_l^i) \Big] - \phi^y
\end{equation}
% \begin{equation}
%         \errc \leq \sum_{(\xv, \xl) \in S} \Bigg[ \sum_{y' \in [r] \setminus \{y(\xv)\}} \sum_{\substack{\xl' \in \Xl^S \\ y(\xl') = j}} A(\xv, \xl') +  \sum_{\substack{\xv' \in \Xv^S \\ y(\xv') = j}} A(\xv', \xl)\Bigg] - \phi^y
% \end{equation}
\end{lemma}
The proof can be found in Appendix 
\ref{app:proof:lemma:errc_bound}.

The subset that minimizes the upper-bound on the conductance error can be found by maximizing the following submodular objective function:
\begin{equation}\label{obj:phi}
    % S^*_{\phi}=
    F_{\phi}(S) = C - \sum_y \sum_{i\in S_y} \sum_{j\in S_{y'\neq y}} \Big[ A(x_v^i,x_l^j)+A(x_v^j,x_l^i) \Big],
\end{equation}
where $C$ is a big constant.

\paragraph{Obtaining Small Labeling Error}
Finally, we discuss finding a subset with a small labeling error.
\begin{lemma}\label{lemma:erra_bound}[labeling error]
For a subset $S \subseteq V$, the labeling error can be calculated as follows:
\begin{equation}
    \erra = C' - \Big(\sum_{i \in V} \At(x_v^i,x_l^i) - \sum_{i \in S} \At(x_v^i,x_l^i) \Big),
\end{equation}
where $C'$ is a constant.
\end{lemma}
The proof can be found in Appendix \ref{app:proof:lemma:erra_bound}.
We see that the subset that minimizes the labeling error can be found by maximizing the following objective function:
\begin{equation}\label{obj:alpha}
    % S^*_{\alpha}\in \argmax_{S \subseteq V, |S|\leq k} 
    F_{\alpha}^S=\sum_{i \in S} \At(x_v^i,x_l^i),
\end{equation}

The above objective selects the examples which have the largest diagonal entries in $\At$.

The above problem is non-monotone submodular, as it is a sum of two non-monotone submodular functions $F_{\sigma}, F_{\phi}$, and a modular function $F_{\alpha}$. Hence, a near-optimal solution can be efficiently computed. \ba{todo: explain alg and guarantee}


\begin{theorem}[Generalization Gap]\label{thm:gen_gap}
    Let $(f_V^*, f_L^*)$ be a minimizer of the loss on full data i.e. $L_{SCL}(f_V, f_L)$ and let $({f_V^S}^*, {f_L^S}^*)$ be a minimizer of the loss on the subset $S$ i.e. $L_{SCL}^S(f_V, f_L)$. Let $\errc \leq \delta_{\errc}$, $\errsv \leq \delta_{\errsv}$ and $\erra \leq \delta_{\erra}$ be the conductance error, the singular value error and the excess labeling error respectively. 

\begin{equation}
    \errlp{{f_V^S}^*} - \errlp{f_V^S} \lesssim \delta_{\errc} + \delta_{\errsv} + \delta_{\erra}
\end{equation}
\end{theorem}
where $\lesssim$ omits some constant terms and finite sample generalization terms. 

Proof in \ref{app:proof:thm:gen_gap}.


\ba{Todo: Zero-shot theorem}

Next, we discuss two practical considerations that often arises when learning from large vision-language datasets.

\paragraph{Dealing with Class Imbalance}
When classes are extremely imbalanced, very large classes dominate $F_{\sigma}$. To prevent this we add the following reguralizer: 
\begin{equation}
    F_{\sigma}^r=F_{\sigma}-\sum_{i\in S} \frac{F_{\sigma}(i)}{|V_y|}
\end{equation}

\paragraph{Label Centrality for Zero-shot Classification}
Since labels are not the center of text classes in practice, we add the following term to encourage selection of examples which has closer text to the labels: \ba{fix}
\begin{equation}
    F_{zs}=\sum_{i\in S} \frac{1}{2}\At(x_l^i,y) - \sum_{i\in S} \frac{\At(x_l^i,y)}{2|V_y|},
\end{equation}
where the second term prevents domination of classes with very good similarity to the label. This improves the zero-shot performance on various datasets.

Final objective:
\begin{equation}\label{eq:final_obj}
    S^*\in\argmax_{S\subset V, |S|\leq k} F^r_{\sigma}(S)+F_{\phi}(S)+2F_{\alpha}(S)+\eta F_{zs}(S),
\end{equation}
where $\eta$ is the average text similarity over average text-to-image similarity.


\begin{comment}
To tractably find the optimal subset $S$ with minimial excess generalization error, we determine the following 3 objectives i.e. minimizing the discrepancy between conductance, the singular values and the labeling error of the subset and that of the full data distribution.

\begin{definition}
Let $\errc$, $\errsv$ and $\erra$ be the conductance error, the singular value error and the excess labeling error, respectively. 

\begin{align}
    &\errc := \phi^y_S - \phi^y_S \\
    &\errsv \ \ :=\sigma_{k+1} - \sigma_{k+1}^S \\
    &\erra := \alpha_y^S - \alpha_y
\end{align}
\end{definition}

Thus, our objective it to minimize $\errc$, $\errsv$ and $\erra$

\sj{When I write not in S, I should clarify I mean not in S but in D. The reason is that I want to distinguish between considering all possible pairs i.e. the universe v/s what is paired in full data v/s what is paired in our subset}



\begin{lemma}\label{lemma:errsv_bound}[\sj{Bounding the singular value error}]
Let $\cross((\xv, \xl)) = \sum_{\xl'} \tilde{A}(\xv, \xl') + \sum_{\xv'} \tilde{A}(\xv', \xl)$

$$\errsv \leq \sum_{(\xv, \xl) \in D} \cross((\xv, \xl)) - \sum_{(\xv, \xl) \in S} \cross((\xv, \xl)) +  \phi^y$$

\sj{make this bound more fine-grained and submodular}
\end{lemma}

Proof in Appendix \ref{app:proof:lemma:errsv_bound}





\begin{lemma}\label{lemma:errc_bound}[\sj{Bounding the conductance error}]
Let $\divit{j} = \sum_{\substack{\xl' \in \Xl^S \\ y(\xl') = j}} A(\xv, \xl')$ and $\divti{j} = \sum_{\substack{\xv' \in \Xv^S \\ y(\xv') = j}} A(\xv', \xl)$

    $$\errc \leq \sum_{(\xv, \xl) \in S} \Bigg[ \sum_{y' \in [r] \setminus \{y(\xv)\}} \divit{y'} + \divti{y'} \Bigg] - \phi^y$$
\end{lemma}

Proof in Appendix \ref{app:proof:lemma:errc_bound}. 


\begin{lemma}\label{lemma:erra_bound}[\sj{Bounding the excess labeling error}]
Let $\selfedge{x} = \pmm(\xv, \xl)$ where $x = (\xv, \xl)$. 

    $$ \erra \approx |S| - \sum_{x \in S} \selfedge{x} - \sum_{x \in D} (1 - \selfedge{x})$$
\end{lemma}

Proof in Appendix \ref{app:proof:lemma:erra_bound}.



To minimize the gap in generalization between training on the full data and the subset, it is sufficient to minimize the aforementioned errors. 


\begin{theorem}\label{thm:error_bound}

Let $\err(S) = \errsv + \errc + \erra$ and let $S_* = \argmin_S \err(S)$

\sj{Modify this and definition of cross to make cross only sum over cross in LC, can do this by showing that -div term cancels that out, so approximately we can not include that. Just need to think about why div term is still there then. Is / should div be 2x according to theory}

$$S_* \approx \argmin_S \Bigg[ -1 \cdot \sum_{(\xv, \xl) \in S} \bigg(\cross((\xv, \xl))  
+  \selfedge{x}
- \sum_{y' \in [r] \setminus \{y(\xv)\}} \divit{y'} + \divti{y'} \bigg)
\Bigg]$$

\end{theorem}

Proof in \ref{app:proof:thm:error_bound}

\sj{Using the above objective, we can find $S$ s.t. $\err(S)$ is minimized and hence we can guarantee that $\errsv$, $\errc$ and $\erra$ are small.} We now provide a guarantee on the downstream generalization performance of the model trained on the subset $S$. 
\end{comment}


\subsection{Finding these subsets efficiently in practice}

Finally, we present our method, \method, which finds subsets that minimize the singular value, conductance and excess labeling errors efficiently. 

\textbf{Approximating the co-occurrence matrix}

Maximizing the objective in Eq. \eqref{eq:final_obj} assumes access to the co-occurrence matrix. To approximate this, we leverage the fact that the product of the image and language representation matrices $F_V F_L^\top$ closely approximate the co-occurrence matrix for trained $f_V$ and $f_L$ \footnote{This follows immediately from Theorem \ref{thm:mmcl=amf}}. We approximate the co-occurrence matrix by constructing image and language representation matrices using pretrained CLIP \citep{pmlr-v139-radford21a}'s models as our proxies $f^p_V$ and $f^p_L$ for the trained vision and language encoder, respectively. \sj{fix: For simplicity, we assume the marginals $\pv$ and $\pl$ over images and captions, respectively, are uniform within every latent class and that every latent class is equally likely. Thus, the diagonal blocks of the approximate normalized co-occurrence matrix can be obtained by simply scaling each block by the size of the cluster. the approximate co-occurrence matrix.}

\textbf{Approximating Latent Classes}

One of the primary strengths of \mmcl is its ability to generalize across a variety of downstream tasks. However, the theoretical guarantees in Theorem \ref{thm:gen_gap} provided theoretical guarantees are with respect to a given downstream task. It is computationally intractable to consider the objective that would explicitly guarantee performance on all possible downstream tasks; instead, we find the subset with respect to the latent classes specified by a fine-grained task e.g. \imgnet \citep{imagenet_cvpr09} as it can ensure that the learnt representations that are discriminative enough for coarser grained tasks as well. However, in practice, we do not even have access to latent classes specified by this fine-grained task. To remedy this, we approximately find our latent classes by using a pretrained CLIP model. In particular, we use zero-shot classification on the images of the dataset with respect to the \imgnet\  labels to partition the dataset into latent classes. We choose to construct partitions only based on images as, in practice, it is difficult to determine latent class membership for most captions as they may not be sufficiently descriptive. \sj{further explain?}

\iffalse
\textbf{Ensuring Captions are Consistent with Labels}

\sj{awk: Theoretically, zero-shot evaluation in done by assigning each image to the text latent class it is closest to in representation space.} However, accurately determining the average similarity with the text latent class is not possible and thus, the similarity to the embedding of the class name is used instead in practice \citep{pmlr-v139-radford21a}. Interestingly, we find that the average embedding of latent classes in text are often not fully aligned with the labels used during zero-shot evaluation \sj{add numbers for this?}. Thus, we also include similarity to ImageNet labels as part of our objective to ensure that the selected are aligned with the labels used by the current zero shot evaluation mechanism. \sj{A recent line of work \citep{an2023context} illustrates the limitations of current zero shot evaluation and resolving these would likely obviate the need for this term.?}
\fi 

%%%%%% SUBMODULAR GUARANTEEES FOR MONOTONE %%%%%%%%%%%%%%%%%%%
\iffalse 
\textbf{Efficiently finding $S$ that minimizes the objective in Theorem \ref{thm:error_bound}}

The objective in Theorem $\ref{thm:error_bound}$ can be turned into maximizing the following monotone submodular\footnote{A set function $F:2^V \rightarrow \mathbb{R}^+$ is \textit{submodular} if $F(e|S)=F(S\cup\{e\}) - F(S) \geq F(T\cup\{e\}) - F(T),$ for any $S\subseteq T \subseteq V$ and $e\in V\setminus T$.  
$F$ is \textit{monotone} if $F(e|S)\geq 0$ for any $e \! \in \! V \! \setminus \! S$ and $S \subseteq V$.} cover problem:
\begin{equation}\label{eq:submodular}
    S_*= \argmax_S \Bigg[\sum_{(\xv, \xl) \in S} \bigg(\cross((\xv, \xl))  
+  \selfedge{x}
- \sum_{y' \in [r] \setminus \{y(\xv)\}} \divit{y'} + \divti{y'} \bigg)
\Bigg]
\end{equation}
\fi

For maximizing a monotone submodular function $F$, the greedy algorithm provides a $(1-1/e)$ approximation guarantee \citep{wolsey1982analysis}. 
The greedy algorithm starts with the empty set $S_0 =\emptyset$, and at each iteration $l$, chooses an element $e\!\in\! \D $ such that %the {marginal utility}
$S_{l} = S_{l-1} \cup\{{\arg\max}_{e\in V} F(e|S_{l-1})\}$. 

The greedy algorithm finds a near-optimal solution of size $\ssize$ in $\mathcal{O}(|\D| \cdot \ssize $$)$ time. This complexity can be reduced to $\mathcal{O}(|\D|)$ by stochastic evaluation \cite{mirzasoleiman2015lazier} and  accelerated further by lazy evaluations \cite{minoux1978accelerated}. Thus, the subset can be found very efficiently.

\begin{algorithm}[t]
\caption{\method: Finding $S_*$}\label{alg}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Dataset $D$, Subset size $\ssize$, proxy encoders: $f_V^p$ and $f_L^p$, 

\STATE \textbf{Output:} Subset $S$
\STATE $\{V_1, ..., V_K \} \leftarrow$ approximate latent classes

\STATE $\approxA \leftarrow 0_{|\D| \times |\D|}$

\FORALL{$\D_k \in \{\D_1, \cdots, \D_K \}$}
    \FORALL{$x_i, x_j \in {\D}$}
        \STATE $({\xv}_i, {\xl}_i) \leftarrow x_i$
        \STATE $({\xv}_j, {\xl}_j) \leftarrow x_j$
        \STATE $\approxA_{i,j} = f_V^p(\xv_i)f_V^p(\xv_i)$
        \STATE $\approxA_{i,j} = f_V^p(\xv_i)f_V^p(\xv_i)$
    \ENDFOR
    \STATE $S \leftarrow \{\}$
    \STATE $F(S) = \sj{going to fill in after notation finalized}$
    \WHILE{$|S| \leq \ssize$}
    \STATE $e \leftarrow \argmax_{e \in \D \setminus S} F(e|S)$
    \STATE $S \leftarrow S \cup \{ e\}$
    \ENDWHILE
\ENDFOR 
\STATE \textbf{return} $S$
\end{algorithmic}
\end{algorithm}


==> old_versions/v1_method.tex <==
\section{\sj{OLD VERSION: Multimodal Subsets that Generalize on Par with the Full Data}}\label{sec:method}
We start by investigating which properties the subset $S$ must satisfy, such that the learned representations on the subset provide a similar downstream linear probe and zero-shot classification error to that of the full data.

\subsection{Background}
Consider the joint data distribution $\pmm(x_v, x_l)$, where $\pmm \in \mathbb{R}^{N_V \times N_L}$ can be formulated a co-occurrence matrix between all visual-language data pairs \cite{pmlr-v202-zhang23an}: 
% such that $\pmm(x_v, x_l)\geq 0, \forall x_v \in [N_V], x_l \in [N_L]$.
%
% As in \cite{pmlr-v202-zhang23an}, we start by formulating the joint distribution $\pmm(x_v, x_l)$ as a co-occurrence matrix $A \in \mathbb{R}^{N_V \times N_L}$ between all images and captions, where 
\begin{equation}
A(x_v, x_l) = \pmm(x_v, x_l) \geq 0, \forall \xv \in \Xv, \forall \xl \in \Xl.
\end{equation}
%%
Contrastive multimodal learning with spectral loss defined in Eq. \ref{eq:spectral} is equivalent to the asymmetric matrix factorization for the normalized co-occurrence matrix
$\tilde{A}$ 
\begin{equation}\label{eq:low-rank}
L_{AMF}(\tilde{F_V}, \tilde{F_L}) := \norm{\tilde{A} - \tilde{F_V} \tilde{ F_L}^\top}^2,
\end{equation}
where ${F_V} \in \mathbb{R}^{N_V \times q}, {F_L} \in \mathbb{R}^{N_L \times q}$ are matrices containing the scaled image and text representations $(F_V)_{x_v}=\sqrt{\pv}f_V(x_v)^T, (F_L)_{x_l}=\sqrt{\pl}f_V(x_l)^T$, computed using the vision and language encoders $f_V, f_L$, and $\tilde{A}$ is the co-occurrence matrix %obtained by performing two-sided normalization 
$\tilde{A}_{\xv, \xl} := \frac{A_{\xv, \xl}}{\sqrt{\pv(\xv) \pl(xl)}}$, normalized by marginal probabilities of image $x_v$, i.e., $\pv(\xv) := \sum_\xv A_{\xv, \xl}$, and text $x_l$, i.e., $\pl(\xl) := \sum_\xl A_{\xv, \xl}$.
% \textbf{\sj{Linear Probe Error}}
% \begin{theorem}[\sj{modified version of Lemma B.1 from \cite{zhang2023generalization}}]\label{thm:lp_error}
% Let $(f_V^*, f_L^*)$ be a minimizer of the population loss $L_{SCL}(f_V, f_L)$

Then, the linear probe error $\errlp{f_V^*}$ for a downstream task with labels $y$ is upper-bounded by:
\begin{equation}
\errlp{f_V^*} \leq \frac{2\phi^y}{1 - \sigma^2_{k+1}} + 8\alpha_y.
\end{equation}
% \end{theorem}
The linear probe error depends on $\sigma_{k+1}$, conductance $\phi$, and labeling error $\alpha$, defined below.

\textbf{Singular values of $\pmb{\tilde{A}}$} $\sigma_1 \geq \cdots \geq \sigma_q$ are singular values of $\tilde{A}$, 
%$\pmb{\sigma_{k+1}}$ is the $k+1^{th}$ largest singular value of $\tilde{A}$ 
capturing the connectivity of the specified by $A$.

Larger singular value of $\tilde{A}$ correspond to better connectivity in the bipartite graph. Better intra-class connectivity leads to more similar representations for images and captions within a latent class.

% and $\phi$ and $\alpha$ are defined as follows:

\textbf{Conductance ($\pmb{\phi}$)} captures the probability of image and text from different classes to co-occur:
\begin{align}
    \phi^y &= \sum_{\xv, xl} \pmm(\xv, \xl) \mathbbm{1}[y(\xv) \neq y(\xl)].
    % \alpha_y &= \E_{\xv, \xl} \mathbbm{1}[{y}(\xv)\neq y(\xl)].
\end{align}

Low conductance corresponds to less inter-class connectivity, which in turn leads to less similar representations for images and captions in different latent classes.

%%%
\textbf{Labeling error $\pmb{\alpha}$} is labeling error capturing discrepancy in labels between the image-caption pairs:
\begin{align}
    % \phi^y &= \sum_{\xv, xl} \pmm(\xv, \xl) \mathbbm{1}[y(\xv) \neq y(\xl)],\\
    \alpha_y &= \E_{\xv, \xl} \mathbbm{1}[{y}(\xv)\neq y(\xl)].
\end{align}

Low labeling error corresponds to low probability that an image and caption are incorrectly paired i.e. the caption does not describe the contents of the image. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Let $y$ be the labeling function associated with a given downstream task s.t. $y(x) := i$ if $x$ belongs to latent class $i$. 

% \begin{definition}[Labeling Error for Task Specified by $y$]
% \begin{equation}
%     \alpha_y = \E_{\xv, \xl} \mathbbm{1}[{y}(\xv)\neq y(\xl)],
% \end{equation}
% \end{definition}

% \begin{definition}[Conductance for Task Specified by $y$]
%     \begin{equation}
%         \phi^y = \sum_{\xv, xl} \pmm(\xv, \xl) \mathbbm{1}[y(\xv) \neq y(\xl)]
%     \end{equation}
% \end{definition}


% \begin{theorem}[ZS error]\label{thm:zs_error}

% $\tilde{F_V}$ are the \sj{normalized?} image and caption representation matrices, respectively i.e. the $\xv$-th row of $\tilde{F_V} = \pv(\xv) \fv{\xv}$ and the $\xl$-th row of $\tilde{F_L} = \pl(\xl) \fl{\xl}$.

% Furthermore, define ${F_V} \in \mathbb{R}^{N_V \times k}$ as the matrix containing the representations of the images, computed using vision encoder $f_V$, i.e. the $\xv$-th row of ${F_V}$ is exactly $\fv{\xv}$. Similarly,  let ${F_L} \in \mathbb{R}^{N_L \times k}$ be the matrix containing the representations of the images, computed using vision encoder $f_L$, i.e. the $\xv$-th row of ${F_L}$ is exactly $\fv{\xl}$. 


% \cite{pmlr-v202-zhang23an} showed that low-rank matrix factorization objective on the normalized co-occurence matrix $\tilde{A}$ $$L_{AMF}(\tilde{F_V}, \tilde{F_L}) := \norm{\tilde{A} - \tilde{F_V} \tilde{ F_L}^\top}^2_F$$ where $\tilde{F_V}$ are the \sj{normalized?} image and caption representation matrices, respectively i.e. the $\xv$-th row of $\tilde{F_V} = \pv(\xv) \fv{\xv}$ and the $\xl$-th row of $\tilde{F_L} = \pl(\xl) \fl{\xl}$. 


\begin{comment}
\textbf{\sj{MMCL = AMF}}
\begin{theorem}[Theorem 3.1 from \cite{pmlr-v202-zhang23an}]\label{thm:mmcl=amf}
\sj{drop?: Let the $\xv$-row of $F_V$ and the
$\xl$-row of $F_L$ represent the corresponding encoded features of these samples in the following form, ${(F_V)}_\xv = \sqrt{\pv_(\xv)} \fv{\xv}^\top$ and ${(F_L)}_\xl = \sqrt{\pl (\xl)} \fl{\xl}^\top$}

Then the low-rank asymmetric matrix factorization loss is equivalent to the multi-modal contrastive loss up to a constant,
$$L_{AMF}(F_V, F_L) = L_{SCL}(f_V, f_L) + const.$$
\end{theorem}

Using this equivalence, \cite{pmlr-v202-zhang23an} proves that the generalization error of multi-modal contrastive learning on a given downstream task can be determined by the labeling error , the conductance and the k+1-th largest singular value of the normalized co-occurrence matrix.

In particular, the downstream generalization errors using linear probe and zeroshot classification can be bound as follows:

% \end{theorem}

\textbf{Labeling error} $\alpha_y$ accounts for the discrepancy in labels between the image-caption pairs, which can vary in practice based on how the dataset is generated.

\textbf{Singular Value} According to the spectral graph theory \cite{chung_1997}, the singular values  represent the connectivity of the bipartite graph specified by $A$. Larger singular value of $\tilde{A}$ correspond to better connectivity. 
\end{comment}


\subsection{Finding Generalizable Multimodal Subsets}
We rely on the above observations to find subsets $S \subset V$ of size $|S|\leq k$ that provide very similar generalization performance to that of the full data, on various downstream tasks. Such subsets should (1) best preserve the singular values $\sigma_i$ of the normalized co-occurrence matrix $\tilde{A}$, (2) have a small conductance $\phi$, and (3) small labeling error $\alpha$. Ensuring (1), (2) and (3) pn the subset $S$, given that every example in $V \setminus S$ is sufficiently similar to an examples in $S$, guarantees good generalization on the entire population. 
% \sj{del?: In addition, to ensure a superior generalization performance on the entire population we also require that (4) the selected subset to be similar to all the examples in $V$.}

Let $M_{R, C}$ be the matrix where $\forall r \in R, \forall c \in C, M_{r, c} = 1$ and 0 everywhere else. 

\begin{lemma}[MMCL on Subset is AMF on Masked $\tilde{A}$]\label{lemma:subset_mmcl}
$\exists$ constant $c$ s.t.

$$c^2 L_{SCL}^S(f_V, f_L) + const. = \norm{M_{S, S} \odot \tilde{A} - F_V F_L^\top}^2$$

\end{lemma}

Proof in Appendix \ref{app:proof:lemma:subset_mmcl}. 

% Since, the generalization performance of multi-modal contrastive learning can be determined by the conductance, the singular value of $\tilde{A}$ and labeling error, a subset that preserves the conductance, connectivity and labeling error of the full data achieves similar generalization performance to the full data. 

\begin{definition}[Cross-Modal Similarity]\label{def:cross_modal_dist}
We define the cross-modal distance between all examples $i, j \in V$ as the sum of the similarity between the representations of the images of examples $i$ and $j$ with the other's caption. Formally, for every pair of examples $i, j \in V$, we have:
\begin{equation}
    \cross{i, j} = \fv{\xv^i} \fl{\xl^j}^\top + \fv{\xv^j} \fl{\xl^i}^\top
\end{equation}
Let the normalized cross-modal distance be
%\begin{equation}
 %   \ncross{i, j} = {\frac{\fv{\xv^i} \fl{\xl^j}^\top}{\sqrt{\pv(\xv^i)}\sqrt{\pl(\xl^j)}}}^2 + {\frac{\fv{\xv^j} \fl{\xl^i}^\top}{\sqrt{\pv(\xv^j)}\sqrt{\pl(\xl^i)}}}^2
%\end{equation}
\end{definition}
\paragraph{Preserving the Spectrum of the Normalized Co-occurrence Matrix}

We start by finding subsets that best preserve the spectrum of the normalized co-occurrence matrix $\tilde{A}$. 

%As shown in Lemma \ref{lemma:subset_mmcl}, training on the subset $S\subset V$ can be modeled as learning representations that recover the masked normalized co-occurrence matrix $M_{S, S} \odot \tilde{A}$. 

%This ensures that the generalization guarantees on the subset extend to the true population. 

%Let $\At_S$ the matrix that captures the masked normalized co-occurrence matrix and the similarities i.e. $$\At_S = M_{S, S} \odot \tilde{A} + \underbrace{M_{S, V \setminus S} \odot \At}_{\text{sim. between image in $S$ and caption in $V \setminus S$}} +  \underbrace{M_{V \setminus S, S} \odot \At}_{\text{sim. between caption in $S$ and image in $V \setminus S$}}$$

Selecting a subset $S\subset V$ can be modeled as perturbing the normalized co-occurrence matrix $\tilde{A}$, where the norm of the perturbation  $\norm{E}=\norm{\tilde{A}-M_{S, S} \odot \tilde{A}}$, is a function of the sum of entries in $\tilde{A}$ that are zeroed out. From \cite{weyl1912asymptotic}, we have that $\errsv = |\sigma'_i - \sigma_i|\leq \norm{E}$, where $\sigma'_i$ and $\sigma_i$ are the singular values of the $M_{S, S} \odot \At$ and original normalized co-occurrence matrix respectively. Therefore, the subset that minimizes the upper-bound of change on the singular values of $\tilde{A}$ is the one that has the smallest norm of error $\norm{E}$, given that every example in $V \setminus S$ is sufficiently similar to an example in $S$. Moreover, $\norm{E} \leq \norm{\At} - \sqrt{\sum_{i \in S} \sum_{j \in S} {\At(x_v^i,x_l^j)}^2 + {\At(x_v^j,x_l^i)}^2}$. Thus, we have the following constrained optimization: 

 \begin{align}\label{eq:errsv_ss}
 \min_S {\norm{F} - \sqrt{\frac{1}{2} \sum_{i \in S} \sum_{j \in S} {\At(x_v^i,x_l^j)}^2 + {\At(x_v^j,x_l^i)}^2}} \nonumber \\ \text{  s.t.   }  \forall i \in V \setminus S, \exists j, \cross{i, j} \geq \boundintra
\end{align} where $\boundintra$ is the minimum sufficient similarity required between for all examples in $V \setminus S$ to an example in $S$ ($\boundintra \approx 2 - o(1)$). 

We use the bound in Eq. \eqref{eq:errsv_ss} and relax the constrained optimization by maximising the similarity between examples in $S$ and those in $V \setminus S$ to get:

\begin{align}
\errsv &= {|\sigma_r  - \sigma_r^S|} \nonumber \\ &\leq \norm{A} - \sqrt{\frac{1}{2} \sum_{i \in S} \sum_{j \in V} {\At(x_v^i,x_l^j)}^2 + {\At(x_v^j,x_l^i)}^2}
\end{align}



%Formally, we wish to solve:
 %\begin{equation}
  %   S^*_{\sigma}\in \argmin \|\tilde{A}-M_S\odot \tilde{A}\|. \quad 
 %\end{equation}

%To bound the error in preserving the spectrum, we rely on Weyl’s theorem \cite{weyl1912asymptotic}
%stating that under bounded perturbations $E$ to a matrix, no singular value can move more than the norm of the perturbations. Formally, $|\sigma'_i - \sigma_i|\leq \norm{E}$, where $\sigma'_i$ and $\sigma_i$ are the singular values of the $M_{S, S} \odot \At$ and original normalized co-occurrence matrix respectively.

%Therefore, the subset that minimizes the upper-bound of change on the singular values of $\tilde{A}$ is the one that has the smallest norm of error $\|E\|$. %Formally, we wish to solve:
%Selecting a subset $S\subset V$ can be modeled as perturbing the normalized co-occurrence matrix $\tilde{A}$, where the norm of the perturbation  $\norm{E}=\norm{\tilde{A}-M_S\odot \tilde{A}}$, is a function of the sum of entries in $\tilde{A}$ that are zeroed out. Therefore, the subset that minimizes the upper-bound of change on the singular values of $\tilde{A}$ is the one that has the smallest norm of error $\|E\|$. %Formally, we wish to solve:
% \begin{equation}
%     S^*_{\sigma}\in \argmin \|\tilde{A}-M_S\odot \tilde{A}\|.
% \end{equation}

% deleted old eq
\iffalse
\begin{equation}
\errsv = {|\sigma_r - \sigma_r^S|}^2 \leq \norm{A} - \sqrt{\frac{1}{2} \sum_{i \in S} \sum_{j \in S} {\At(x_v^i,x_l^j)}^2 + {\At(x_v^j,x_l^i)}^2}  \quad \forall r\in[q]   
\end{equation}
\fi

% deleted section on intra-class connectivity
\iffalse
\textbf{Ensuring sufficient intra-class connectivity between $S$ and $V \setminus S$}

To guarantee good generalization on the true population, we need the vision and language encoders trained on the subset to preserves the similarities between the representations of $S$ and $V \setminus S$ in every latent class. 
Let $\errcc$ be defined as the intra-class connectivity between $S$ and $V$ i.e. $\errc = \frac{1}{2} \sum_{i \in S_y}\sum_{j \in V_y \setminus S_y}  {\At(x_v^i,x_l^j)}^2 + {\At(x_v^j,x_l^i)}^2$
\fi

\begin{lemma}[Approximating Singular Value Error with Cross Modal Similarities]\label{lemma:approx_errsv}
$$\argmin_S \errc \approx \argmax_S \sum_{i \in S} \sum_{j \in V} \cross{i, j}$$
\end{lemma}

Proof in Appendix \ref{proof:lemma:approx_errsv}. 

Thus we have that the subset that minimizes the error on the singular values can be found as well by maximizing the following monotone submodular\footnote{A set function $F : 2^V \rightarrow \mathbb{R}^+$ is submodular if $F(e|S) = F(S \cup \{e\})-F(S) \geq F(T \cup \{e\})-F(T)$, for any $S \subseteq T \subseteq V$ and $e \in V \setminus T$. $F$ is monotone if $F(e|S) \geq 0$ for any $e \in V \setminus S$
and $S \subseteq V$.} function

\begin{equation}\label{obj:sigma}
    F_{\sigma}(S) = \sum_{i \in S} \sum_{j\in V} \cross{i, j}
\end{equation}

The subset that maximizes the above objective covers the largest entries of $\At$. Approximately, this objective selects examples that maximize cross modal similarity $\cross{}$ to the whole data i.e. these examples have captions that co-occur with many images and images that co-occur with many captions. This enables \mmcl\ to bring the representations of different examples closer together, as effectively as the full data, despite training on the subset. 

\paragraph{Achieving Small Conductance}

To find subsets with small conductance, we need to minimize the cross-modal similarity between images and text in different classes.

For any subset $S \subseteq V$, and a given labeling $y$, the difference between the 
conductance of the subset $\phi_S^y$ and full data is: 
% \begin{equation}
%     % \errc = \phi^y - \phi^y_S
%     % \leq \phi^y -
%     F_{\phi}(S)=\phi_S^y= \sum_{\substack{\xv \in \Xv^S \\ \xl \in \Xl^S}} \mathbbm{1}[y(\xv) \neq y(\xl)] A(\xv,\xl).
% \end{equation}

% Note that $S \subset \Xv^S \times \Xl^S$

% old 15, which is not the definition, so this is not an equality: 
% \begin{equation}
%     % \errc = \phi^y - \phi^y_S
%     % \leq \phi^y -
%     F_{\phi}(S)=\phi_S^y= \sum_{\substack{(\xv, \xl) \in S}} \mathbbm{1}[y(\xv) \neq y(\xl)] A(\xv,\xl).
% \end{equation}
\begin{equation}
        \errc = \phi_S^y -\phi^y = \sum_y \sum_{i\in S_y} \sum_{j\in S_{y'\neq y}} \Big[ \cross{i, j} \Big] - \phi^y
\end{equation}

Moreover, to guarantee good generalization on the full data, we must also satisfy the constraint that examples in $S_y$ do not have large cross-modal similarity to examples in $V \setminus S_y$ i.e.

\begin{equation}\label{eq:errc_constraint}
    \forall y, \sum_{i \in S_y} \sum_{j \in V \setminus S_y} \cross{i, j} \leq \boundinter
\end{equation}

We relax this constrained optimization problem by minimizing, $\forall y$, the similarity between examples in $S_y$ and those in $V \setminus S_y$. Thus, the subset that minimizes the conductance error while satisfying constraint \eqref{eq:errc_constraint}.

%\begin{equation}
 %       \errc = \phi_S^y -\phi^y \leq \sum_y \sum_{i\in S_y} \sum_{j\in S_{y'\neq y}} \Big[ \frac{\cross{i, j}}{|S_{y' \neq y}|} \Big] - \phi^y
%\end{equation}
% \begin{equation}
%         \errc \leq \sum_{(\xv, \xl) \in S} \Bigg[ \sum_{y' \in [r] \setminus \{y(\xv)\}} \sum_{\substack{\xl' \in \Xl^S \\ y(\xl') = j}} A(\xv, \xl') +  \sum_{\substack{\xv' \in \Xv^S \\ y(\xv') = j}} A(\xv', \xl)\Bigg] - \phi^y
% \end{equation}
 

\begin{equation}\label{obj:phi}
    % S^*_{\phi}=
    F_{\phi}(S) = C - \sum_y \sum_{i\in S_y} \sum_{j\in V \setminus S_y} \Big[ \cross{i, j} \Big],
\end{equation}
where $C$ is a big constant.

The subset that maximizes this objective contains examples that have smallest cross-modal similarity to examples in other latent classes. This is what enables \mmcl\ to push apart representations of examples in different latent classes, as effectively as the full data, despite training on the subset.

\paragraph{Obtaining Small Labeling Error}

Finally, we discuss finding a subset with a small labeling error.

For a subset $S \subseteq V$, the excess labeling error can be calculated as follows:
\begin{equation}
    \erra = \sum_{i \in V} \frac{\cross{i, i}}{2} - \sum_{i \in S} \frac{\cross{i, i}}{2},
\end{equation}

We see that the subset that minimizes the labeling error can be found by maximizing the following objective function:
\begin{equation}\label{obj:alpha}
    % S^*_{\alpha}\in \argmax_{S \subseteq V, |S|\leq k} 
    F_{\alpha}^S= \sum_{i \in S} \cross{i, i},
\end{equation}.



The above objective selects the examples which have the largest diagonal entries in $A$. This ensures that, with high probability, the image-captions pairs in $S$ are correctly matched i.e the image and caption belong to the same latent class. This effectively prevents selecting examples whose image and caption are prioritizing high cross-modal similarity to different latent classes.

The subsets that (1) best preserve the singular values $\sigma_i$ of the normalized co-occurrence matrix  $\At$, (2) have a small conductance $\phi$, and (3) small labeling error $\alpha$ can be found by maximizing the objectives in Eq. \ref{obj:sigma}, \ref{obj:phi}, \ref{obj:alpha}: 
\begin{equation}\label{eq:obj}
    S^* = \argmax_{S\subset V, |S|\leq k} F_{\sigma}(S) + F_{\phi}(S) + F_{\alpha}(S).
\end{equation}



%The above problem is non-monotone submodular, as it is a sum of two non-monotone submodular functions $F_{\sigma}, F_{\phi}$, and a modular function $F_{\alpha}$. Hence, a near-optimal solution can be efficiently computed. \ba{todo: explain alg and guarantee}



\begin{theorem}[Generalization Gap]\label{thm:gen_gap}
    Let $(f_V^*, f_L^*)$ be a minimizer of the loss on full data i.e. $L_{SCL}(f_V, f_L)$ and let $({f_V^S}^*, {f_L^S}^*)$ be a minimizer of the loss on the subset $S$ i.e. $L_{SCL}^S(f_V, f_L)$. Let $\errc \leq \delta_{\errc}$, $\errsv \leq \delta_{\errsv}$ and $\erra \leq \delta_{\erra}$ be the conductance error, the singular value error and the excess labeling error respectively. Given that   $\forall i \in V \setminus S, \exists j, \cross{i, j} \geq \boundintra$ for $\boundintra$ sufficiently large and $\forall y, \sum_{i \in S_y} \sum_{j \in V \setminus S_y} \cross{i, j} \leq \boundinter$ for for $\boundinter$ sufficiently small.
\begin{equation}
    \errlp{{f_V^S}^*} - \errlp{f_V^S} \lesssim \delta_{\errc} + \delta_{\errsv} + \delta_{\erra}
\end{equation}

and 

\begin{equation}
    \errzs{{f_V^S}^*} - \errzs{f_V^S} \lesssim \delta_{\errc} + \delta_{\errsv} + \delta_{\erra}
\end{equation}

\end{theorem}
where $\lesssim$ omits some constant terms and finite sample generalization terms. 


Proof in \ref{app:proof:thm:gen_gap}.

Next, we discuss two practical considerations that often arises when learning from large vision-language datasets.

\paragraph{Dealing with Class Imbalance}

When classes are extremely imbalanced, very large classes dominate $F_{\sigma}$. To prevent this, we normalize the terms in $F_{\sigma}$ corresponding to each latent class $y \in [\numclasses]$ by the size of latent classes $|V_y|$. Moreover, to avoid overly biasing towards latent classes that have much higher intra-class cross-modal similarity than others,  we add further regularization. 

In summary,

\begin{equation}\label{eq:regularize_fphi}
    F_{\sigma}^r=  \sum_{y \in [\numclasses]} \sum_{i \in S_y} \sum_{j\in V} \underbrace{\frac{\cross{i, j}}{|V_y|}}_{\text{normalization}} - \underbrace{\frac{\cross{i, j}}{|V_y|^2}}_{\text{regularization}}
\end{equation}

To ensure that the $F_{\sigma}$ and $F_{\phi}$ are of similar scale, we normalize terms in $F_{\phi}$ as well by the size of the corresponding latent classes i.e 
\begin{equation}\label{eq:regularize_fphi}
    F_{\phi}^r = \sum_{\substack{y,y' \in [\numclasses] \\ y \neq y'}} \sum_{i \in S_y} \sum_{j \in V_y'}\frac{\cross{i, j}}{|V_y|}
\end{equation}

\paragraph{Label Centrality for Zero-shot Classification}
Since labels are not the center of text classes in practice, we add the following term to encourage selection of examples which has closer text to the labels:
\begin{equation}
    F_{zs}=\sum_{i\in S} \frac{1}{2}\At(x_l^i,y) - \sum_{i\in S} \frac{\At(x_l^i,y)}{2|V_y|},
\end{equation}
where the second term prevents domination of classes with very good similarity to the label. This improves the zero-shot performance on various datasets.

 Finally, in order to allow for $F_{\sigma}$,  $F_{\phi}$ and $F_{\alpha}$ to be minimized equally, we scale $F_\alpha$ by a factor of 2. 


\begin{remark}\label{remark:simple_obj}
    \begin{align}
    &\argmax_{S\subset V, |S|\leq k} F^r_{\sigma}(S)+F_{\phi}(S)+2F_{\alpha}(S)+\eta F_{zs}(S)  \\
    &\approx \argmax_{S\subset V, |S|\leq k} \underbrace{\sum_{y \in [\numclasses]} \sum_{i \in S_y} \sum_{j \in V_y} \frac{\cross{i, j}}{|V_y|}}_{\text{intra-class cross-modal similarity}} \nonumber \\ &- \underbrace{\sum_{\substack{y,y' \in [\numclasses] \\ y \neq y'}} \sum_{i \in S_y} \sum_{j \in V_y'}\frac{\cross{i, j}}{|V_y|}}_{\text{inter-class cross-modal similarity}} + \underbrace{\sum_{i \in S} \cross{i, i}}_{\text{cross-modal self similarity}} 
    \nonumber \\ &-  \underbrace{\sum_{y \in [\numclasses]} \sum_{i \in S_y} \sum_{j \in V_y} \frac{\cross{i, j}}{|V_y|^2}}_{\text{intra-class cross-modal regularization}} - \underbrace{\eta F_{zs}(S)}_{\text{label centrality}}
    \end{align}
where $\eta$ is the average text similarity over average text-to-image similarity.
\end{remark}

Proof in Appendix \ref{app:proof:remark:simple_obj}. 

In Fig. \ref{fig:obj_matrix}, we visualize the different components of the objective (omitting the regularization and label-centrality terms for simplicity). We show in this figure that the objective in Remark \ref{remark:simple_obj} selects a subsets that preserves the intra-class cross-modal similarity as well as the cross-modal self-similarity while minimizing the inter-class cross-modal similarity.

%Thus, the final objective is: 

%\begin{equation}\label{eq:final_obj}
%    S^* = \argmax_{S\subset V, |S|\leq k} F^r_{\sigma}(S)+F_{\phi}(S)+2F_{\alpha}(S)+\eta F_{zs}(S),
%\end{equation}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/obj_matrix.pdf}
    \caption{Visualization of the Objective in Remark \ref{remark:simple_obj} (blue represents terms the objective wants to maximize and red/pink represents terms the objective wants to minimize}
    \label{fig:obj_matrix}
\end{figure*}

\begin{comment}
To tractably find the optimal subset $S$ with minimial excess generalization error, we determine the following 3 objectives i.e. minimizing the discrepancy between conductance, the singular values and the labeling error of the subset and that of the full data distribution.

\begin{definition}
Let $\errc$, $\errsv$ and $\erra$ be the conductance error, the singular value error and the excess labeling error, respectively. 

\begin{align}
    &\errc := \phi^y_S - \phi^y_S \\
    &\errsv \ \ :=\sigma_{k+1} - \sigma_{k+1}^S \\
    &\erra := \alpha_y^S - \alpha_y
\end{align}
\end{definition}

Thus, our objective it to minimize $\errc$, $\errsv$ and $\erra$

\sj{When I write not in S, I should clarify I mean not in S but in D. The reason is that I want to distinguish between considering all possible pairs i.e. the universe v/s what is paired in full data v/s what is paired in our subset}



\begin{lemma}\label{lemma:errsv_bound}[\sj{Bounding the singular value error}]
Let $\cross((\xv, \xl)) = \sum_{\xl'} \tilde{A}(\xv, \xl') + \sum_{\xv'} \tilde{A}(\xv', \xl)$

$$\errsv \leq \sum_{(\xv, \xl) \in D} \cross((\xv, \xl)) - \sum_{(\xv, \xl) \in S} \cross((\xv, \xl)) +  \phi^y$$

\sj{make this bound more fine-grained and submodular}
\end{lemma}

Proof in Appendix \ref{app:proof:lemma:errsv_bound}





\begin{lemma}\label{lemma:errc_bound}[\sj{Bounding the conductance error}]
Let $\divit{j} = \sum_{\substack{\xl' \in \Xl^S \\ y(\xl') = j}} A(\xv, \xl')$ and $\divti{j} = \sum_{\substack{\xv' \in \Xv^S \\ y(\xv') = j}} A(\xv', \xl)$

    $$\errc \leq \sum_{(\xv, \xl) \in S} \Bigg[ \sum_{y' \in [r] \setminus \{y(\xv)\}} \divit{y'} + \divti{y'} \Bigg] - \phi^y$$
\end{lemma}

Proof in Appendix \ref{app:proof:lemma:errc_bound}. 


\begin{lemma}\label{lemma:erra_bound}[\sj{Bounding the excess labeling error}]
Let $\selfedge{x} = \pmm(\xv, \xl)$ where $x = (\xv, \xl)$. 

    $$ \erra \approx |S| - \sum_{x \in S} \selfedge{x} - \sum_{x \in D} (1 - \selfedge{x})$$
\end{lemma}

Proof in Appendix \ref{app:proof:lemma:erra_bound}.



To minimize the gap in generalization between training on the full data and the subset, it is sufficient to minimize the aforementioned errors. 


\begin{theorem}\label{thm:error_bound}

Let $\err(S) = \errsv + \errc + \erra$ and let $S_* = \argmin_S \err(S)$

\sj{Modify this and definition of cross to make cross only sum over cross in LC, can do this by showing that -div term cancels that out, so approximately we can not include that. Just need to think about why div term is still there then. Is / should div be 2x according to theory}

$$S_* \approx \argmin_S \Bigg[ -1 \cdot \sum_{(\xv, \xl) \in S} \bigg(\cross((\xv, \xl))  
+  \selfedge{x}
- \sum_{y' \in [r] \setminus \{y(\xv)\}} \divit{y'} + \divti{y'} \bigg)
\Bigg]$$

\end{theorem}

Proof in \ref{app:proof:thm:error_bound}

\sj{Using the above objective, we can find $S$ s.t. $\err(S)$ is minimized and hence we can guarantee that $\errsv$, $\errc$ and $\erra$ are small.} We now provide a guarantee on the downstream generalization performance of the model trained on the subset $S$. 
\end{comment}


\subsection{Finding \method\ Subsets Efficiently from Large Data}

In this section, we discuss how \method can be efficiently implemented to extract subsets with superior generalization performance from very large image-caption datasets.
% minimize the singular value, conductance and excess labeling errors efficiently. 
Specifically, we discuss approximation the co-occuerence probabilities \ba{example similarities}, how to find the latent classes, and how to extract the subsets efficiently from large datasets.

\textbf{Approximating the co-occurrence matrix}

%Maximizing the objective in Eq. \eqref{eq:final_obj} requires access to the co-occurrence probabilities. To approximate this, we leverage the fact that the co-occurrence matrix $A$ can be calculated as $\At(x_v,x_l)=\left<f_V(x_v),f_L(x_l)\right>\sqrt{\pv(x_v)\pl(x_l)}$, where $f_V$ and $f_L$ are vision and language encoders trained with the CLIP loss and $\pv(x_v),\pl(x_l)$ are marginal probabilities of image $x_v$ and text $x_l$, respectively. Assuming all the $c$ latent classes are equally likely and all examples in a latent class are equally likely, we can approximate the marginal probability for a given example $(x_v,x_l)\in V_y$ in class $y$ as $\pv(x_v)=\pl(x_l)={1}/{c|V_y|}$. Using a pre-trained CLIP model with vision and language encoders $f_V^p, f_L^p$ as a proxy, we estimate the co-occurrence probability for an example $(x_v,x_l)$ in latent class $y$ as $\At(x_v,x_l)=\left<f_V^p(x_v),f_L^p(x_l)\right>/c|V_y|$. 
Maximizing the objective in Remark \ref{remark:simple_obj} requires access to the co-occurrence probabilities. To approximate this, we leverage the fact that the co-occurrence matrix $A$ can be calculated as $\A(x_v,x_l)=\left<f_V(x_v),f_L(x_l)\right>$, where $f_V$ and $f_L$ are vision and language encoders trained with the CLIP loss, respectively. Using a pre-trained CLIP model with vision and language encoders $f_V^p, f_L^p$ as a proxy, we estimate the co-occurrence probability for an example $(x_v,x_l)$ as $A(x_v,x_l)=\left<f_V^p(x_v),f_L^p(x_l)\right>$. That is, the co-occurrence probability for an example can be estimated as the the cosine similarity of its image-caption representations according to a pre-trained CLIP.

% the product of the image and language representation matrices $F_V F_L^\top$ closely approximate the normalized co-occurrence matrix $\At$ according to Eq. \eqref{eq:low-rank}, where $(F_V)_{x_v}=\sqrt{\pv(x_v)}f_V(x_v)^T$ and $(F_L)_{x_l}=\sqrt{\pl(x_l)}f_V(x_l)^T$, and vision and language encoders $f_V$ and $f_L$ are trained with the CLIP loss. We use image and language encoders $f^p_V$ and $f^p_L$ of a pretrained CLIP model, and rely on the assumption that 
% as the size of the dataset grow very large, images have an equal marginal probability $\pv$ to exist in the data. The same argument holds for the marginal probability of captions $\pl$.
% all the latent classes are equally likely, we approximate the marginal probability for every image or caption in latent class $y$ by $\sqrt{\pv(x_v)}=\sqrt{\pv(x_l)}=1 / (c \times |V_c|)$, where $c$ is the number of latent classes.

% Based on this observation, we approximate the normalized co-occurrence probabilities as the cosine similarity of the image and language representations obtained using 
% That is $\At(x_v^i)=\left< f_V^p(x_v^i), f_L^p(x_l^i) \right>$. 

% \sj{fix: For simplicity, we assume the marginals $\pv$ and $\pl$ over images and captions, respectively, are uniform within every latent class and that every latent class is equally likely. Thus, the diagonal blocks of the approximate normalized co-occurrence matrix can be obtained by simply scaling each block by the size of the cluster. the approximate co-occurrence matrix.}

\textbf{Approximating Latent Classes}
The objective in Remark \ref{remark:simple_obj} requires that 
a partitioning of the data w.r.t labels of the downstream task is given at the time of pre-training.
% the class labels are known for all the examples in the dataset. 
However, the  downstream task(s) and their labels are not known at the time of pre-training. Besides, even if the set of relevant labels are known, such labeling for all the examples in the large pre-training data is not provided. 
Crucially, we wish the pre-trained model to generalize to a variety of downstream tasks. 
Nevertheless, if one can label all the training examples with a \textit{large set of fine-grained labels}, the pre-trained model with a good generalization w.r.t the fine-grained labels will also have a good performance w.r.t various course-grained labeling of the data.  
% To address this, we chose a large pool of fine-grained labels and label the pre-training examples. 
We achieve this by using the zero-shot classification ability of a pre-trained CLIP model to label all the images of the training data with the \imgnet \cite{imagenet_cvpr09} labels. We partition the image-caption pairs into different classes only based on their images as, in practice, the class for a given caption containing different words may be ambiguous.

% One of the primary strengths of \mmcl is its ability to generalize across a variety of downstream tasks. However, the theoretical guarantees in Theorem \ref{thm:gen_gap} provided theoretical guarantees are with respect to a given downstream task. It is computationally intractable to consider the objective that would explicitly guarantee performance on all possible downstream tasks; instead, we find the subset with respect to the latent classes specified by a fine-grained task e.g. \imgnet \cite{imagenet_cvpr09} as it can ensure that the learnt representations that are discriminative enough for coarser grained tasks as well. However, in practice, we do not even have access to latent classes specified by this fine-grained task. To remedy this, we approximately find our latent classes by using a pretrained CLIP model. In particular, we use zero-shot classification on the images of the dataset with respect to the \imgnet\  labels to partition the dataset into latent classes. We choose to construct partitions only based on images as, in practice, it is difficult to determine latent class membership for most captions as they may not be sufficiently descriptive. \sj{further explain?}

\iffalse
\textbf{Ensuring Captions are Consistent with Labels}

\sj{awk: Theoretically, zero-shot evaluation in done by assigning each image to the text latent class it is closest to in representation space.} However, accurately determining the average similarity with the text latent class is not possible and thus, the similarity to the embedding of the class name is used instead in practice \cite{pmlr-v139-radford21a}. Interestingly, we find that the average embedding of latent classes in text are often not fully aligned with the labels used during zero-shot evaluation \sj{add numbers for this?}. Thus, we also include similarity to ImageNet labels as part of our objective to ensure that the selected are aligned with the labels used by the current zero shot evaluation mechanism. \sj{A recent line of work \cite{an2023context} illustrates the limitations of current zero shot evaluation and resolving these would likely obviate the need for this term.?}
\fi 

%%%%%% SUBMODULAR GUARANTEEES FOR MONOTONE %%%%%%%%%%%%%%%%%%%
\iffalse 
\textbf{Efficiently finding $S$ that minimizes the objective in Theorem \ref{thm:error_bound}}

The objective in Theorem $\ref{thm:error_bound}$ can be turned into maximizing the following monotone submodular\footnote{A set function $F:2^V \rightarrow \mathbb{R}^+$ is \textit{submodular} if $F(e|S)=F(S\cup\{e\}) - F(S) \geq F(T\cup\{e\}) - F(T),$ for any $S\subseteq T \subseteq V$ and $e\in V\setminus T$.  
$F$ is \textit{monotone} if $F(e|S)\geq 0$ for any $e \! \in \! V \! \setminus \! S$ and $S \subseteq V$.} cover problem:
\begin{equation}\label{eq:submodular}
    S_*= \argmax_S \Bigg[\sum_{(\xv, \xl) \in S} \bigg(\cross((\xv, \xl))  
+  \selfedge{x}
- \sum_{y' \in [r] \setminus \{y(\xv)\}} \divit{y'} + \divti{y'} \bigg)
\Bigg]
\end{equation}
\fi

\textbf{Scaling to Massive Datasets}
\ba{modify if non-monotone} Dividing the pre-training dataset to fine-grained classes improves the scalability of \method\ to larger datasets, by reducing the complexity of calculating Eq. \eqref{obj:sigma}. Nevertheless, finding the optimal solution for Problem \ref{remark:simple_obj} is NP hard as it requires calculating the objective for an exponential number of subsets. Fortunately, as Problem \ref{remark:simple_obj} is monotone submodular, a near-optimal solution can be found efficiently.
% The objective in Eq. \eqref{eq:final_obj} 
For maximizing a monotone submodular function $F$, the greedy algorithm provides a $(1-1/e)$ approximation guarantee \cite{wolsey1982analysis}. 
The greedy algorithm starts with the empty set $S_0 =\emptyset$, and at each iteration $t$, chooses an element $i\!\in\! V $ such that %the {marginal utility}
$S_{t} = S_{t-1} \cup\{{\arg\max}_{i\in V} F(e|S_{t-1})\}$. The complexity of the greedy algorithm to find $k$ out of $n$ example is $\mathcal{O}(n \cdot k $$)$. This complexity can be reduced to $\mathcal{O}(V)$ by stochastic evaluation \cite{mirzasoleiman2015lazier} and  accelerated further by lazy evaluations \cite{minoux1978accelerated}. Moreover, it scales to millions of data points with distributed \cite{mirzasoleiman2013distributed} and streaming methods \cite{badanidiyuru2014streaming}. Thus, the subset can be found very efficiently from massive multimodal datasets.

The pseudocode of \method\ is illustrated in Alg. \ref{alg}.

\begin{algorithm}[t]
\caption{\method: Finding $S_*$}\label{alg}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Dataset $V$, Subset size $\ssize$, proxy encoders: $f_V^p$ and $f_L^p$, 

\STATE \textbf{Output:} Subset $S$
\STATE $\{V_1, ..., V_K \} \leftarrow$ approximate latent classes

\STATE $\approxA \leftarrow 0_{|\D| \times |\D|}$

\FORALL{$\D_k \in \{\D_1, \cdots, \D_K \}$}
    \FORALL{$x_i, x_j \in {\D}$}
        \STATE $({\xv}_i, {\xl}_i) \leftarrow x_i$
        \STATE $({\xv}_j, {\xl}_j) \leftarrow x_j$
        \STATE $\approxA_{i,j} = f_V^p(\xv_i)f_V^p(\xv_i)$
        \STATE $\approxA_{i,j} = f_V^p(\xv_i)f_V^p(\xv_i)$
    \ENDFOR
    \STATE $S \leftarrow \{\}$
    \STATE $F(S)$ := as defined in Remark. \ref{remark:simple_obj}
    \WHILE{$|S| \leq \ssize$}
    \STATE $e \leftarrow \argmax_{e \in \D \setminus S} F(e|S)$
    \STATE $S \leftarrow S \cup \{ e\}$
    \ENDWHILE
\ENDFOR 
\STATE \textbf{return} $S$
\end{algorithmic}
\end{algorithm}


==> old_versions/v2_method.tex <==
\section{Multimodal Subsets that Generalize on Par with the Full Data}\label{sec:method}

In this section, we investigate which properties the subset $S$ must satisfy, such that the learned representations on the subset provide a similar downstream linear probe and zero-shot classification error to that of the full data. In particular, we start by introducing generalization guarantees for models trained on the full data. We then utilize these guarantees to provide generalization guarantees for models trained on the subset $S$. Finally, we show how to minimize the gap between generalization error on the subset $S$  and the full data. 

\subsection{Preliminaries}

For ease of theoretical analysis, the spectral multi-modal contrastive loss is often used \cite{pmlr-v202-zhang23an} in place of the CLIP loss. Fundamentally, both the CLIP loss and the spectral multi-modal contrastive loss bring representations of paired image-captions closer together while pushing apart representations of unpaired image-captions. \sj{del?: and yield a similar performance in visual tasks \cite{haochen2022provable}}.
\begin{align}\label{eq:spectral}
    \mathcal{L}_{SCL}(f_V, f_L) = -2 \E_{x_v, x_l \sim \pmm} f_V(x_v)^\top f_L(x_l)\nonumber \\ + \E_{\substack{x_v^- \sim \pv \\ x_l^- \sim \pl}} {(f_V(x_V^-)^\top f_L(x_l^-)})^2.
\end{align}

The joint data distribution $\pmm(x_v, x_l)$, can be formulated a co-occurrence matrix $A\in \mathbb{R}^{N_V \times N_L}$ between all visual-language data pairs \cite{pmlr-v202-zhang23an}:

\begin{equation}\label{eq:co-occurence_mtx}
A(x_v, x_l) = \pmm(x_v, x_l) \geq 0, \forall \xv \in \Xv, \forall \xl \in \Xl.
\end{equation}

Contrastive multimodal learning with the spectral loss defined in Eq. \ref{eq:spectral} is equivalent to asymmetric matrix factorization (AMF) for the normalized co-occurrence matrix 
$\tilde{A}$ \cite{pmlr-v202-zhang23an}:
\begin{equation}\label{eq:amf}
L_{AMF}(\tilde{F_V}, \tilde{F_L}) := \norm{\tilde{A} - \tilde{F_V} \tilde{ F_L}^\top}^2,
\end{equation}
where ${F_V} \in \mathbb{R}^{N_V \times q}, {F_L} \in \mathbb{R}^{N_L \times q}$ are matrices containing the scaled image and text representations $(F_V)_{x_v}=\sqrt{\pv}f_V(x_v)^T, (F_L)_{x_l}=\sqrt{\pl}f_V(x_l)^T$, computed using the vision and language encoders $f_V, f_L$, and $\tilde{A}$ is the co-occurrence matrix %obtained by performing two-sided normalization 
$\tilde{A}_{\xv, \xl} := \frac{A_{\xv, \xl}}{\sqrt{\pv(\xv) \pl(xl)}}$, normalized by marginal probabilities of image $x_v$, i.e., $\pv(\xv) := \sum_\xv A_{\xv, \xl}$, and text $x_l$, i.e., $\pl(\xl) := \sum_\xl A_{\xv, \xl}$.

Intuitively, this shows the probability of $\xv$ and $\xl$ co-occurring i.e. $\pmm(\xv, \xl)$ is approximately the similarity of representations of $\xv$ and $\xl$ obtained using encoders $f_\mathcal{V}$ and $f_\mathcal{L}$, respectively.

Then, \cite{pmlr-v202-zhang23an} shows that the linear probe error $\errlp{f_V^*}$ for this downstream task is upper-bounded by:
\begin{equation}\label{eq:lp_zhang}
\errlp{f_V^*} \leq \frac{2\phi^y}{1 - \sigma^2_{k+1}} + 8\alpha_y.
\end{equation}

\begin{equation}
   \errlp{f_V^*} \leq \phi_{lp}(\text{intra-class}, \text{labeling error})
\end{equation}
% \end{theorem}
where $\sigma_{k+1}$, conductance $\phi$, and labeling error $\alpha$ are as defined here:

Let $\{ V_{y} \}_{y \in \mathcal{Y}}$ be the latent classes specified by $\mathcal{Y}$ i.e. the labels of the given downstream task. 

\textbf{Singular values of $\pmb{\tilde{A}}$} $\sigma_1 \geq \cdots \geq \sigma_q$ are singular values of $\tilde{A}$. The singular vectors and values of $\tilde{A}$ capture the patterns in co-occurrence of images and captions representations.\sj{More concretely, larger $\sigma_{k+1}$ corresponds to higher probability of co-occurrence for images and captions within latent classes. Larger $\sigma_{k+1}$ corresponds to lower generalization error as shown in Eq. \eqref{eq:lp_zhang}}

%\sj{For example, captions containing "a dog" are quite likely to co-occur with many different images in the dog latent class. Likewise, an image containing "a dog" are likely to co-occur with many captions in the dog latent class. This high probability of co-occurrence within the dog latent class would contribute to larger singular values for the corresponding $\tilde{A}$.}

\textbf{Conductance ($\pmb{\phi}$)} captures the probability that images from two different latent classes are paired with the same caption:
\begin{align}
    &\phi^y := \\&\sum_{\substack{\xv \in \Xv \\ \xv' \in \Xv}} \underset{\xl \in \Xl}{\mathbb{E}} \pmm(\xv | \xl) \pmm(\xv' | \xl) \mathbbm{1}[y(\xv) \neq y(\xv')].
\end{align}
 
Hence, low conductance corresponds to low likelihood of images from different latent classes being paired with the same caption. \sj{For example, an image of "a dog and a person" and an image of "a cat and a person" that belong to the dog and cat latent classes, respectively, are both likely to be paired with captions containing "a person". Such examples would lead to high conductance, which is undesirable. In contrast, an image of only "a dog" and an image of only "a cat" are more unlikely to be paired with same caption. This would lead to low conductance, which is desirable.}

\textbf{Labeling error $\pmb{\alpha}$} is the probability that a given image-caption pair is incorrectly paired together:
%i.e. the image and caption belong to different latent classes:
\begin{align}
    \alpha_y &= \E_{\xv, \xl \sim \pmm} \mathbbm{1}[{y}(\xv)\neq y(\xl)].
\end{align}

\sj{Intuitively, if for most image-caption pairs, the caption accurately describes what is in the image, labeling error is low.}

%%%%% GRAPH EXPLANATION %%%%%%%%%

 %To better understand the effects of the aforementioned terms, consider the weighted bipartite graph specified by $A$ as an adjacency matrix i.e $\Xv, \Xl$ are the vertex sets and the weight of the edge between $\xv \in \Xv$ and $\xl \in \Xl$ is $A(\xv, \xl)$. Additionally, let the labels $y$ of the downstream task specify the latent classes. The \textit{singular values of $\tilde{A}$} capture the connectivity of this bipartite graph. Larger singular values correspond to more connectivity in this bipartite graph; this leads to representation within  

Since objective \eqref{eq:problem_formulation} requires subsets that achieve low linear probe and zero-shot classification error, we first provide generalization guarantees for zero-shot classification. 

\begin{lemma}[Zero-Shot Classification Generalization Error]
For vision encoder $f_\mathcal{V}$ and language encoder $f_\mathcal{L}$, the generalization error of zero-shot classification can be bounded as follows:
\begin{align}
\errzs{f_\mathcal{V}^*, f_\mathcal{L}^*} \leq \mathcal{O}(\phi^y + \sigma_{k+1})
\end{align}
where $\phi^y$ is the conductance and $\sigma_{k+1}$ is the k+1-th largest singular value of the normalized co-occurrence matrix $\tilde{A}$.
\end{lemma}

\begin{equation}
   \errzs{f_V^*, f_L^*} \leq \phi_{zs}(\text{intra-class}, \text{labeling error}, \text{label sim})
\end{equation}

\sj{Proof in Appendix}.

\subsection{Characterizing the most Generalizable Subset}

%We now utilize the aforementioned bounds for generalization on the full data to provide bounds for generalization on the subset $S$. 

Here, we first utilize the aforementioned bounds for generalization on the full data to determine the generalization error for training on any subset $S \subset V$. Then, we use the generalization guarantee on arbitrary subsets $S$ to characterize $S_*$ i.e. the generalizable subset.

\begin{definition}[Normalized Co-occurrence Matrix for the Subset $S$] \label{def:}
Let $M_{R, C}$ be the matrix where $\forall r \in R, \forall c \in C, M_{r, c} = 1$ and 0 everywhere else. Then, $\tilde{A}^S$, the normalized co-occurrence matrix for the subset $S$ is defined as:
$$\tilde{A}_S = M_{S, S} \odot \tilde{A}$$
\end{definition}

\begin{lemma}[MMCL on Subset $S$ is Equivalent AMF on  $\tilde{A}_S$]\label{lemma:subset_mmcl}
$\exists$ constant $c$ s.t.

$$c^2 L_{SCL}^S(f_V, f_L) + const. = \norm{\tilde{A}_S - F_V F_L^\top}^2$$
\end{lemma}

\sj{Proof in Appendix.}

Let $\tau$ be the fraction of examples in $V_y \setminus S_y$ that are, on average, are sufficiently to co-occur with examples in $S_y$ i.e. for these examples, \sj{images co-occur often enough with captions and captions occur often enough with images.}

\begin{theorem}[Generalization Error on Subset $S$]\label{thm:gen_err_subset} For vision encoder $f_\mathcal{V}^S$ and language encoder $f_\mathcal{L^S}$ trained on the subset $S$, the generalization error of linear probe can be bounded as such: 
\begin{align}
    \errlp{f_\mathcal{V}^S} \leq \frac{2\phi^y}{1 - \sigma^2_{k+1}} + 8\alpha_y + (1 - \tau)
\end{align}
and the generalization error of zero-shot classification can be bounded as such:
\begin{align}
    \errzs{f_\mathcal{V}^S, f_\mathcal{L}^S} \leq \mathcal{O}(\phi^y + \sigma_{k+1}) + (1 - \tau)
\end{align}

where $\phi^y_S$ is the conductance on the subset, $\sigma_{k+1}^S$ is the k+1-th largest singular value of $\tilde{A}_S$ i.e. the normalized co-occurrence matrix for the subset $S$ and $\alpha_y^S$ is the labeling error of the subset.
\end{theorem}

The subset $S_*$ that satisfies Objective \eqref{eq:problem_formulation} is characterized in Corollary \ref{corr:gen_gap} that follows from Theorem \ref{thm:gen_err_subset}.

\begin{corollary}\label{corr:gen_gap}
Let $S^* = \argmin_{S\subseteq V, |S|\leq n_s} \delta_{lp} + \delta_{zs}$ (Objective \eqref{eq:problem_formulation}). 

\begin{align}
S_* = \argmin \errsv + \errc + \erra + (1 - \tau)
\end{align}
where $\errsv = | \sigma_{k+1}^S - \sigma_{k+1} |$, $\errc = \phi^y_S - \phi^y$  and $\erra = \alpha_y^S - \alpha_y$ i.e. the change in conductance, singular values of normalized co-occurrence matrix and labeling error, between the subset $S$ and the full data, respectively.
\end{corollary}

\subsection{Finding the most Generalizable Subset}

%\sj{sketch:1. define cross-modal sim i j and remark that i j cross modal similarity is equal to i j probability of co-occurrence. 2. SV error -> S-S 3. conductance error -> approximate by minimizing sim to center 4. labeling error  5. maximize $\tau$ 6. putting it together and simplifying, theorem.  7. state what intra-class cross-modal similarity, inter-class cross-modal similarity and cross-modal self-similarity are and explain how this ensures pairs are not mislabeled and representations of examples. 8. to deal with class imbalance, we add regularization. then present final objective.}

Using the characterization of generalizable subsets in Corollary \ref{corr:gen_gap}, we now show how to find such subsets \sj{using the representations of any vision and language encoder $f_{\mathcal{V}}$ and $f_{\mathcal{L}}$, trained using the spectral multimodal contrastive loss}.

\sj{We want to approximate $\pmm$ since we don't have access to the distribution.} 

since the AMF loss (Eq. \eqref{eq:amf}) is equivalent to the spectral loss, for trained vision and language encoders $f_\mathcal{V}$ and $f_\mathcal{L}$, 
\begin{align}\label{eq:observation}
    \pmm(\xv^i, \xl^j) + \pmm(\xv^j, \xl^i) \approx \cross{i, j}
\end{align} 

\sj{have 2 equations, 1 for each pm term}

\begin{definition}[Cross-Modal Similarity]\label{def:cross_modal_dist}

We define the cross-modal distance between all examples $i, j \in V$ as the sum of the similarities between the representations of the images of examples $i$ and $j$ with the other's caption. Formally, for every pair of examples $i, j \in V$, we have:
\begin{equation}
    \cross{i, j} = \fv{\xv^i} \fl{\xl^j}^\top + \fv{\xv^j} \fl{\xl^i}^\top
\end{equation}
\end{definition}

\tilde{sim}

Using the observation in Eq. \eqref{eq:observation}, we now discuss how to minimize $\errsv, \errc, \erra$ i.e. the difference in singular values, conductance and labeling error between the subset $S$ and the full data, as well as $(1 - \tau)$ i.e the fraction of examples that do not co-occur sufficiently with the subset $S$. 

\textbf{Preserving the Spectrum of the Normalized Co-occurrence Matrix}

To minimize  $\errsv = | \sigma_{k+1}^S - \sigma_{k+1} - |$, $\tilde{A}_S$, the normalized co-occurrence matrix for the subset $S$ should preserve the spectrum of $\tilde{A}$, the normalized co-occurrence matrix for the full data. From \cite{weyl1912asymptotic}, we have that, $\forall i, |\sigma_i^S - \sigma_i| \leq \norm{E}$ where $E = \tilde{A}_S - \tilde{A}$. 

Hence, $\errsv \leq \sqrt{\norm{E}^2} = \sqrt{\sum_{\substack{i \in S \\ j \in S}} \tilde{A_{ij}}^2 + \tilde{A_{ji}}^2 } - const.$ where $const. = \sum_{\substack{i \in V \\ j \in V}} \tilde{A_{ij}}^2 + \tilde{A_{ji}}^2$ is independent of the subset $S$. 

\sj{show both cases $S_y$to itself and $S$toitself} Additionally, it is easy to see that preserving the likelihood of images and captions in different latent classes co-occurring is undesirable. Concretely, this would worsen generalization on the subset due to higher conductance and labeling error. Thus, we only optimize to preserve co-occurrence probabilities within latent classes. Finally, in order to approximate the normalized co-occurrence matrices $\tilde{A}_S$ and $\tilde{A}$ using cross-modal similarity, we must normalize the cross-modal similarities by the marginal probability distributions as in Eq. \eqref{eq:amf}. We approximate this normalization using the size of latent classes\sj{, implicitly assuming that every latent class is equally likely and within latent classes every example is equally likely.} \footnote{Appendix \ref{app:proof:lemma:errsv} illustrates in detail why this is a reasonable approximation.}
Formally,

\begin{lemma}[Minimizing Singular Value Error using Cross-Modal Similarities]\label{lemma:errsv}
$$\argmin_S \errsv \approx \argmax_S F_\sigma(S)$$

where $F_\sigma(S) = \sum_{i \in S_y, j \in S_y,  y \in \mathcal{Y}} \frac{\cross{i, j}}{|V_y|}$
\end{lemma}

\sj{Proof in Appendix.}

Intuitively, this corresponds to a subset $S$ where all images and captions in the subset, within a given latent class, have representations that are very similar. \sj{repeat intuitive explanation?}

\textbf{Achieving Small Conductance}

To minimize $\errc$, images in different latent classes in the subset $S$ should not be paired with the same caption. However, would require $N_\mathcal{V} \cdot N_{\mathcal{L}}$ similarity computations, which is extremely expensive. Thus, we approximate this using the sum of similarities of images representations to the average caption representation of other latent classes and similarities of caption representations to the average image representation of the the other latent classes. Ensuring the aforementioned similarities are small implies that image representations from distinct latent classes $y_i$ and $y_j$ cannot both be similar to caption representations in latent class $y_k$, thus the image representations cannot be similar to same caption representation.
Formally, 
\begin{lemma}[Minimizing Conductance Difference using Cross-Modal Similarity]\label{lemma:errc}
$$\argmin_S \errc \approx \argmin_S F_\phi(S) $$

where $F_\phi(S) :=  \sum_{\substack{i \in S_y \\ j \in S_{y'} \\ y \neq y'}} \cross{i, j}$.
\end{lemma}

\sj{Proof in Appendix. For consistency in notation, we express the cross-modal similarity to the average representation of the class in terms of the pairwise cross-modal similarities.}

\paragraph{Obtaining Small Labeling Error}

To minimize $\erra = \alpha_y^S - \alpha_y$, it is sufficient to ensure that image-caption pairs in $S$ are correctly paired together i.e. the caption describes the contents of the image. The probability that an image and caption both capture the same objects is often estimated by the similarity of the image \cite{gadre2023datacomp} i.e. the cross-modal similarity of an example to itself.

\begin{lemma}[Minimizing Excess Labeling Error using Cross-Modal Similarities]\label{lemma:erra}
 $$argmin_S \erra F_{\alpha}(S)$$

where $F_\alpha(S) = \sum_{i \in S} \cross{i, i}$
\end{lemma}

\sj{Proof in Appendix.} 

\textbf{Minimizing $1 - \tau(S)$ \sj{/  the fraction of examples in $V_y \setminus S_y$ that are not likely to co-occur with examples in $S_y$}}

To minimize $(1 - \tau(S))$, we must ensure that the representations of images and captions of examples in $V_y \setminus S_y$, i.e. the examples from latent class $V_y$ that are not in $S$ are similar to the representations of examples in $S_y$ i.e. examples selected from latent class $V_y$. 

\begin{lemma}[Minimizing $1 - \tau(S)$ using Cross-Modal Similarities]\label{lemma:tau}
    $$\argmin_S 1 - \tau(S) \approx \argmax F_\tau(S)$$ where
    $F_\tau(S) = \sum_{\substack{i \in S_y // j \in V_y \setminus S_y // y \in \mathcal{Y}}} \cross{i, j}$
\end{lemma}

\textbf{\sj{better title: Combining the objectives}}

Combining the objective functions from Lemmas \ref{lemma:errsv}, \ref{lemma:errc}, \ref{lemma:erra} and \ref{lemma:tau}, we show in Theorem \ref{thm:obj} the objective that can be used to \textbf{find generalizable subsets.} 

\begin{theorem}[Finding Generalizable Subsets]\label{thm:obj} The subset $S_*$ that minimizes both linear probe and zero-shot classification generalization can be found by approximating the following objective: 
\begin{align}
    &\argmin_{S\subseteq V, |S|\leq n_s} \delta_{lp} + \delta_{zs}\\
    &= \argmin_S \errsv + \errc + \erra + (1 - \tau(S)) \nonumber\\ 
    &\text{using Corollary \ref{corr:gen_gap}}\\
    &\approx \argmin_S F_\sigma(S) + F_\phi(S) + F_\alpha(S) + F_\tau(S) \nonumber\\ 
    &\text{using Lemmas \ref{lemma:errsv}, \ref{lemma:errc} \ref{lemma:erra} \ref{lemma:tau}} \\
    &= \argmax_S F(S)
\end{align}
where 
\begin{align}
F(S) &:=  \underbrace{\sum_{y \in [\numclasses]} \sum_{i \in S_y} \sum_{j \in V_y} \frac{\cross{i, j}}{|V_y|}}_{\text{intra-class cross-modal similarity}} \nonumber \\ &- \underbrace{\sum_{\substack{y,y' \in [\numclasses] \\ y \neq y'}} \sum_{i \in S_y} \sum_{j \in S_y'}\frac{\cross{i, j}}{|V_y'|}}_{\text{inter-class cross-modal similarity}}  + \underbrace{\sum_{i \in S} \cross{i, i}}_{\text{cross-modal self similarity}} 
    \nonumber 
\end{align}
\end{theorem}

\sj{Proof in Appendix.} \sj{explanation of what kind of subset this is and reference figure.}


\sj{From here on, haven't reworked yet, but will keep mostly same:}

Next, we discuss two practical considerations that often arises when learning from large vision-language datasets.

\paragraph{Dealing with Class Imbalance}

When classes are extremely imbalanced, very large classes dominate $F_{\sigma}$. To prevent this, we normalize the terms in $F_{\sigma}$ corresponding to each latent class $y \in [\numclasses]$ by the size of latent classes $|V_y|$. Moreover, to avoid overly biasing towards latent classes that have much higher intra-class cross-modal similarity than others,  we add further regularization. 

In summary,

\begin{equation}\label{eq:regularize_fphi}
    F_{\sigma}^r=  \sum_{y \in [\numclasses]} \sum_{i \in S_y} \sum_{j\in V} \underbrace{\frac{\cross{i, j}}{|V_y|}}_{\text{normalization}} - \underbrace{\frac{\cross{i, j}}{|V_y|^2}}_{\text{regularization}}
\end{equation}

To ensure that the $F_{\sigma}$ and $F_{\phi}$ are of similar scale, we normalize terms in $F_{\phi}$ as well by the size of the corresponding latent classes i.e 
\begin{equation}\label{eq:regularize_fphi}
    F_{\phi}^r = \sum_{\substack{y,y' \in [\numclasses] \\ y \neq y'}} \sum_{i \in S_y} \sum_{j \in V_y'}\frac{\cross{i, j}}{|V_y|}
\end{equation}

\paragraph{Label Centrality for Zero-shot Classification}
Since labels are not the center of text classes in practice, we add the following term to encourage selection of examples which has closer text to the labels:
\begin{equation}
    F_{zs}=\sum_{i\in S} \frac{1}{2}\At(x_l^i,y) - \sum_{i\in S} \frac{\At(x_l^i,y)}{2|V_y|},
\end{equation}
where the second term prevents domination of classes with very good similarity to the label. This improves the zero-shot performance on various datasets.

 Finally, in order to allow for $F_{\sigma}$,  $F_{\phi}$ and $F_{\alpha}$ to be minimized equally, we scale $F_\alpha$ by a factor of 2. 


\begin{remark}\label{remark:simple_obj}
    \begin{align}
    &\argmax_{S\subset V, |S|\leq k} F^r_{\sigma}(S)+F_{\phi}(S)+2F_{\alpha}(S)+\eta F_{zs}(S)  \\
    &\approx \argmax_{S\subset V, |S|\leq k} \underbrace{\sum_{y \in [\numclasses]} \sum_{i \in S_y} \sum_{j \in V_y} \frac{\cross{i, j}}{|V_y|}}_{\text{intra-class cross-modal similarity}} \nonumber \\ &- \underbrace{\sum_{\substack{y,y' \in [\numclasses] \\ y \neq y'}} \sum_{i \in S_y} \sum_{j \in V_y'}\frac{\cross{i, j}}{|V_y|}}_{\text{inter-class cross-modal similarity}} + \underbrace{\sum_{i \in S} \cross{i, i}}_{\text{cross-modal self similarity}} 
    \nonumber \\ &-  \underbrace{\sum_{y \in [\numclasses]} \sum_{i \in S_y} \sum_{j \in V_y} \frac{\cross{i, j}}{|V_y|^2}}_{\text{intra-class cross-modal regularization}} - \underbrace{\eta F_{zs}(S)}_{\text{label centrality}}
    \end{align}
where $\eta$ is the average text similarity over average text-to-image similarity.
\end{remark}

Proof in Appendix \ref{app:proof:remark:simple_obj}. 



==> old_versions/v2_method_practical.tex <==
\section{ \method\ : Finding Generalizable Subsets Efficiently from Large Data}

\sj{In this section, we discuss how subsets optimizing the objective in  can be efficiently implemented} to extract subsets with superior generalization performance from very large image-caption datasets.
% minimize the singular value, conductance and excess labeling errors efficiently. 
Specifically, we discuss approximation the co-occuerence probabilities \ba{example similarities}, how to find the latent classes, and how to extract the subsets efficiently from large datasets.

\textbf{Approximating the co-occurrence matrix}

%Maximizing the objective in Eq. \eqref{eq:final_obj} requires access to the co-occurrence probabilities. To approximate this, we leverage the fact that the co-occurrence matrix $A$ can be calculated as $\At(x_v,x_l)=\left<f_V(x_v),f_L(x_l)\right>\sqrt{\pv(x_v)\pl(x_l)}$, where $f_V$ and $f_L$ are vision and language encoders trained with the CLIP loss and $\pv(x_v),\pl(x_l)$ are marginal probabilities of image $x_v$ and text $x_l$, respectively. Assuming all the $c$ latent classes are equally likely and all examples in a latent class are equally likely, we can approximate the marginal probability for a given example $(x_v,x_l)\in V_y$ in class $y$ as $\pv(x_v)=\pl(x_l)={1}/{c|V_y|}$. Using a pre-trained CLIP model with vision and language encoders $f_V^p, f_L^p$ as a proxy, we estimate the co-occurrence probability for an example $(x_v,x_l)$ in latent class $y$ as $\At(x_v,x_l)=\left<f_V^p(x_v),f_L^p(x_l)\right>/c|V_y|$. 
Maximizing the objective in Remark \ref{remark:simple_obj} requires access to the co-occurrence probabilities. To approximate this, we leverage the fact that the co-occurrence matrix $A$ can be calculated as $\A(x_v,x_l)=\left<f_V(x_v),f_L(x_l)\right>$, where $f_V$ and $f_L$ are vision and language encoders trained with the CLIP loss, respectively. Using a pre-trained CLIP model with vision and language encoders $f_V^p, f_L^p$ as a proxy, we estimate the co-occurrence probability for an example $(x_v,x_l)$ as $A(x_v,x_l)=\left<f_V^p(x_v),f_L^p(x_l)\right>$. That is, the co-occurrence probability for an example can be estimated as the the cosine similarity of its image-caption representations according to a pre-trained CLIP.

% the product of the image and language representation matrices $F_V F_L^\top$ closely approximate the normalized co-occurrence matrix $\At$ according to Eq. \eqref{eq:low-rank}, where $(F_V)_{x_v}=\sqrt{\pv(x_v)}f_V(x_v)^T$ and $(F_L)_{x_l}=\sqrt{\pl(x_l)}f_V(x_l)^T$, and vision and language encoders $f_V$ and $f_L$ are trained with the CLIP loss. We use image and language encoders $f^p_V$ and $f^p_L$ of a pretrained CLIP model, and rely on the assumption that 
% as the size of the dataset grow very large, images have an equal marginal probability $\pv$ to exist in the data. The same argument holds for the marginal probability of captions $\pl$.
% all the latent classes are equally likely, we approximate the marginal probability for every image or caption in latent class $y$ by $\sqrt{\pv(x_v)}=\sqrt{\pv(x_l)}=1 / (c \times |V_c|)$, where $c$ is the number of latent classes.

% Based on this observation, we approximate the normalized co-occurrence probabilities as the cosine similarity of the image and language representations obtained using 
% That is $\At(x_v^i)=\left< f_V^p(x_v^i), f_L^p(x_l^i) \right>$. 

% \sj{fix: For simplicity, we assume the marginals $\pv$ and $\pl$ over images and captions, respectively, are uniform within every latent class and that every latent class is equally likely. Thus, the diagonal blocks of the approximate normalized co-occurrence matrix can be obtained by simply scaling each block by the size of the cluster. the approximate co-occurrence matrix.}

\textbf{Approximating Latent Classes}
The objective in Remark \ref{remark:simple_obj} requires that 
a partitioning of the data w.r.t labels of the downstream task is given at the time of pre-training.
% the class labels are known for all the examples in the dataset. 
However, the  downstream task(s) and their labels are not known at the time of pre-training. Besides, even if the set of relevant labels are known, such labeling for all the examples in the large pre-training data is not provided. 
Crucially, we wish the pre-trained model to generalize to a variety of downstream tasks. 
Nevertheless, if one can label all the training examples with a \textit{large set of fine-grained labels}, the pre-trained model with a good generalization w.r.t the fine-grained labels will also have a good performance w.r.t various course-grained labeling of the data.  
% To address this, we chose a large pool of fine-grained labels and label the pre-training examples. 
We achieve this by using the zero-shot classification ability of a pre-trained CLIP model to label all the images of the training data with the \imgnet \cite{imagenet_cvpr09} labels. We partition the image-caption pairs into different classes only based on their images as, in practice, the class for a given caption containing different words may be ambiguous.

% One of the primary strengths of \mmcl is its ability to generalize across a variety of downstream tasks. However, the theoretical guarantees in Theorem \ref{thm:gen_gap} provided theoretical guarantees are with respect to a given downstream task. It is computationally intractable to consider the objective that would explicitly guarantee performance on all possible downstream tasks; instead, we find the subset with respect to the latent classes specified by a fine-grained task e.g. \imgnet \cite{imagenet_cvpr09} as it can ensure that the learnt representations that are discriminative enough for coarser grained tasks as well. However, in practice, we do not even have access to latent classes specified by this fine-grained task. To remedy this, we approximately find our latent classes by using a pretrained CLIP model. In particular, we use zero-shot classification on the images of the dataset with respect to the \imgnet\  labels to partition the dataset into latent classes. We choose to construct partitions only based on images as, in practice, it is difficult to determine latent class membership for most captions as they may not be sufficiently descriptive. \sj{further explain?}

\iffalse
\textbf{Ensuring Captions are Consistent with Labels}

\sj{awk: Theoretically, zero-shot evaluation in done by assigning each image to the text latent class it is closest to in representation space.} However, accurately determining the average similarity with the text latent class is not possible and thus, the similarity to the embedding of the class name is used instead in practice \cite{pmlr-v139-radford21a}. Interestingly, we find that the average embedding of latent classes in text are often not fully aligned with the labels used during zero-shot evaluation \sj{add numbers for this?}. Thus, we also include similarity to ImageNet labels as part of our objective to ensure that the selected are aligned with the labels used by the current zero shot evaluation mechanism. \sj{A recent line of work \cite{an2023context} illustrates the limitations of current zero shot evaluation and resolving these would likely obviate the need for this term.?}
\fi 

%%%%%% SUBMODULAR GUARANTEEES FOR MONOTONE %%%%%%%%%%%%%%%%%%%
\iffalse 
\textbf{Efficiently finding $S$ that minimizes the objective in Theorem \ref{thm:error_bound}}

The objective in Theorem $\ref{thm:error_bound}$ can be turned into maximizing the following monotone submodular\footnote{A set function $F:2^V \rightarrow \mathbb{R}^+$ is \textit{submodular} if $F(e|S)=F(S\cup\{e\}) - F(S) \geq F(T\cup\{e\}) - F(T),$ for any $S\subseteq T \subseteq V$ and $e\in V\setminus T$.  
$F$ is \textit{monotone} if $F(e|S)\geq 0$ for any $e \! \in \! V \! \setminus \! S$ and $S \subseteq V$.} cover problem:
\begin{equation}\label{eq:submodular}
    S_*= \argmax_S \Bigg[\sum_{(\xv, \xl) \in S} \bigg(\cross((\xv, \xl))  
+  \selfedge{x}
- \sum_{y' \in [r] \setminus \{y(\xv)\}} \divit{y'} + \divti{y'} \bigg)
\Bigg]
\end{equation}
\fi

\textbf{Scaling to Massive Datasets}
\ba{modify if non-monotone} Dividing the pre-training dataset to fine-grained classes improves the scalability of \method\ to larger datasets, by reducing the complexity of calculating Eq. \eqref{obj:sigma}. Nevertheless, finding the optimal solution for Problem \ref{remark:simple_obj} is NP hard as it requires calculating the objective for an exponential number of subsets. Fortunately, as Problem \ref{remark:simple_obj} is monotone submodular, a near-optimal solution can be found efficiently.
% The objective in Eq. \eqref{eq:final_obj} 
For maximizing a monotone submodular function $F$, the greedy algorithm provides a $(1-1/e)$ approximation guarantee \cite{wolsey1982analysis}. 
The greedy algorithm starts with the empty set $S_0 =\emptyset$, and at each iteration $t$, chooses an element $i\!\in\! V $ such that %the {marginal utility}
$S_{t} = S_{t-1} \cup\{{\arg\max}_{i\in V} F(e|S_{t-1})\}$. The complexity of the greedy algorithm to find $k$ out of $n$ example is $\mathcal{O}(n \cdot k $$)$. This complexity can be reduced to $\mathcal{O}(V)$ by stochastic evaluation \cite{mirzasoleiman2015lazier} and  accelerated further by lazy evaluations \cite{minoux1978accelerated}. Moreover, it scales to millions of data points with distributed \cite{mirzasoleiman2013distributed} and streaming methods \cite{badanidiyuru2014streaming}. Thus, the subset can be found very efficiently from massive multimodal datasets.

The pseudocode of \method\ is illustrated in Alg. \ref{alg}.

\begin{algorithm}[t]
\caption{\method: Finding $S_*$}\label{alg}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Dataset $V$, Subset size $\ssize$, proxy encoders: $f_V^p$ and $f_L^p$, 

\STATE \textbf{Output:} Subset $S$
\STATE $\{V_1, ..., V_K \} \leftarrow$ approximate latent classes

\STATE $\approxA \leftarrow 0_{|\D| \times |\D|}$

\FORALL{$\D_k \in \{\D_1, \cdots, \D_K \}$}
    \FORALL{$x_i, x_j \in {\D}$}
        \STATE $({\xv}_i, {\xl}_i) \leftarrow x_i$
        \STATE $({\xv}_j, {\xl}_j) \leftarrow x_j$
        \STATE $\approxA_{i,j} = f_V^p(\xv_i)f_V^p(\xv_i)$
        \STATE $\approxA_{i,j} = f_V^p(\xv_i)f_V^p(\xv_i)$
    \ENDFOR
    \STATE $S \leftarrow \{\}$
    \STATE $F(S)$ := as defined in Remark. \ref{remark:simple_obj}
    \WHILE{$|S| \leq \ssize$}
    \STATE $e \leftarrow \argmax_{e \in \D \setminus S} F(e|S)$
    \STATE $S \leftarrow S \cup \{ e\}$
    \ENDWHILE
\ENDFOR 
\STATE \textbf{return} $S$
\end{algorithmic}
\end{algorithm}



==> old_versions/v2_problem_formulation.tex <==
\section{Problem Formulation}

\textbf{{Data  Distribution}}
Let $\mathcal{D}=\{(x_v^i,x_l^i)\}_{i\in V}\sim\pmm$ be a set of $n=|V|$ image-caption pairs, where $x_v^i\in \mathcal{X_V}$ denotes the image and $x_l^i\in \mathcal{X_L}$ denotes the caption of example $i$, and $\pmm$ is the joint multimodal distribution. We denote by $\mathcal{X_V}\sim \mathcal{P_V}$, and $\mathcal{X_L}\sim \mathcal{P_L}$ the set of all images and captions, respectively.
%, where $N_V = |\mathcal{X_V}|$ and $N_L = |\mathcal{X_L}|$. 
We assume each example $(x_v^i,x_l^i)$ belong to one of the $r$ latent classes. 

\textbf{Contrastive Language-Image Pre-training (CLIP)}
CLIP learns image and text embeddings in a shared $k$-dimensional latent space $\mathcal{Z} \in \mathbb{R}^k$, by learning vision encoder $f_V:\mathcal{X_V} \rightarrow \mathcal{Z}$ and language encoder $f_L:\mathcal{X_L} \rightarrow \mathcal{Z}$ by maximizing the similarity between image and caption representations of the same example $(\xv,\xl)\sim\pmm$, and minimizing that of different examples $\xv^-\in\mathcal{P_V}$, $x_l^-\in\mathcal{P_L}$. 
% such that semantically similar examples have close representations and different samples have far away representations. 
The CLIP loss, referred to also as the symmetric cross entropy (SCE) loss is defined as follows:
\begin{align}
    \!\!\mathcal{L}_{SCE}(f_V, f_L) \!=\!
    -\!\!\E_{\xv, \xl \sim \pmm} \!\log \frac{\exp(\fv{\xv}^\top \fl{\xl})}{\E_{\xl^-} \exp(\fv{\xv}^\top \fl{x_l^-})} \nonumber \\
    -\!\! \E_{\xv, \xl \sim \pmm} \!\log \frac{\exp(\fv{\xv}^\top \fl{\xl}}{\E_{\xv^-} \exp(\fv{\xv^-}^\top \fl{\xl})}.
\end{align}

\iffalse
\textbf{{Evaluation}} After training, the quality of the learned representations are evaluated by linear probe and zero-shot classification on various downstream image classification tasks. For a given downstream image classification task, let $\mathcal{Y} = \{y_i\}_{i=1}^r$ be the set of labels and $y(\xv)$ represent the label for example $\xv$. For both evaluations, we first obtain the image representations using the vision encoder $f_\mathcal{V}$. 

\textbf{Linear Probe Error} For linear probe, we train a linear classifier on the encoded representations such that the classification for an example $\xv$ is $g_{f_V,W}(x) := \argmax_{i \in [r]} {(\fv{x}^\top W)}_i$, where $W \in \mathbb{R}^{k \times r}$ is the weight of the trained linear classifier. The linear probing error of $f_V$ is defined as the error of the optimal linear classifier on the encoded representations of the downstream data:

\begin{equation}
\errlp{f_V} := \min_{W \in \mathbb{R}^{k \times r}} \prob{\xv \in \Xv}{y(\xv) \neq g_{f, W}(\xv)}.
\end{equation}

\textbf{Zero-shot Classification Error} For zero-shot classification, we use the language encoder $f_\mathcal{L}$ to encode the labels; then, the classification of an example $\xv$ is $zs_{f_V, f_L}(\xv) = \argmax_{i \in [r]} \frac{\fv{\xv} \cdot z_i}{\norm{\fv{\xv}}\norm{z_i}}$,
where $z_i = \fl{y_i}$ is the language representation of the label. The zero-shot error of $f_V, f_L$ is defined as the fraction of misclassified examples using the trained vision and language encoders $f_V, f_L$:
\begin{equation}
\errzs{f_V, f_L} := \prob{\xv \in \Xv}{y(\xv) \neq zs_{f_V, f_L}(\xv)}.
\end{equation}
% \end{definition}

In practice, for a label $y_i$, \cite{pmlr-v139-radford21a} proposed using a set of pre-engineered templates, e.g. "\texttt{A photo of a \{label\}}" for zero-shot classification. The language representation of the label is then the average of the template language representations.

\textbf{Finding Generalizable Multimodal
Subsets} Our goal is to find a subset $S\subseteq V$ with size at most $n_S \leq n$ that achieves a similar or superior zero-shot and linear probe error compared to that of the encoders trained on the full data. Formally,
\begin{equation}\label{eq:problem_formulation} S^* = \argmin_{S\subseteq V, |S|\leq n_s} \delta_{lp} + \delta_{zs},
\end{equation}
where $\delta_{lp}=|\errlp{f_V}-\errlp{f_V^S}|$ and $\delta_{zs}=|\errzs{f_V, f_L}-\errzs{f_V^S, f_L^S}|$.


% \begin{definition}
% [Zeroshot classification for a given labeling function $y$]
% Average text embedding of class centers specified by $y$:
% $Z = \begin{bmatrix}
%     | & \cdots & | \\
%     \mathbf{z}_1 &  \cdots & \mathbf{z}_r \\ 
%     | & \cdots & |
% \end{bmatrix}$

==> problem_formulation_old.tex <==
% \vspace{-3mm}
\section{PROBLEM FORMULATION}
% \vspace{-3mm}
\textbf{Data Distribution}
% Let $(\xv, \xl) \sim \Dpop$ be an image-caption pair in the population data $\Dpop$ where $\xv$
% denotes the image and $\xl$ denotes the caption. Moreover, let $\Dv_{pop}$ be the set of images and $\Dl_{pop}$ be the set of captions in the population. Let the population data $\Dpop$ be partitioned into $K$ latent classes i.e. $\Dpop = \bigcup_{k \in [K]} \Dpop^k$.
Let $\mathcal{D}=\{(\xv^i, \xl^i)\}_{i\in V}$ be a set of $n=|V|$ image-caption pairs i.e. the full training data available to us, where $\xv^i$ denotes the image and $\xl^i$ denotes the caption of $i$-th example. Moreover, let $\Dv$ be the set of images and $\Dl$ be the set of captions in $\D$. To model the notion that paired image-captions describe the same underlying object, let image-caption pair $(\xv^i, \xl^i) \in \D$ be generated as follows:
\begin{align}
&\xv^i = \Uv (\uf^i + \noisev) \quad\quad \xl^i = \Ul (\uf^i + \noisel),
\end{align} where $\uf^i \in \mathbb{R}^d$ is the shared underlying feature vector for example $i$; $\Uv: \mathbb{R}^d \rightarrow \mathbb{R}^{\dv}$ and  $\Ul: \mathbb{R}^d \rightarrow \mathbb{R}^{\dl}$ are the mappings from underlying feature space to the vision and language data spaces; and $\noisev, \noisel$ are the noise in underlying features for vision and language, respectively. We refer to $\ufnv^i = \uf^i + \noisev^i$ and $\ufnl^i = \uf^i + \noisel^i$ as the noisy underlying feature for the image and caption of example $i$. The underlying feature $\uf^i$, for each image-caption pair is sampled independently of other pairs and of the noise $\noisev, \noisel$. Additionally, we assume $\forall i, \norm{\ufnv}^i, \norm{\ufnl}^i$ and $\norm{\Uv}, \norm{\Ul}$ is $\leq 1$. 
%\sj{To model the notion that image-caption pairs in same latent class describe the same concept and those in different latent classes describe different concepts, we assume that $\forall i, j \in \Dpop^k$, the cosine similarity between $\uf^i$ and $\uf^j = 1$ and $\forall$ distinct $k_1, k_2 \in [K]$, $\forall i \in \Dpop^{k_1}, \forall j \in \Dpop^{k_2}$, the cosine similarity between $\uf^i$ and $\uf^j$ = 0.} 
\sj{Introduce notion of latent class here.}
Similar to prior work \cite{pmlr-v202-xue23d, xue2024investigating, xue2024understanding}, we have that the $k$-th coordinate of the underlying feature vector corresponds to the underlying feature of latent class $k$. \ba{what if two latent classes share a feature? e.g. grass in cat and dog classes.}\sj{if a class has more than 1 feature, you can just think of the feature for that class being the linear combination of them in this theoretical setup.}\ba{this is not what I asked, I said what if they share? then covarianc for them is not zero.} This data-distribution is identical to the data-distribution in \cite{pmlr-v206-nakada23a} to study multi-modal contrastive learning, with the sole addition of latent-classes.
\ba{what's the relation between $d, K$? very confusing!}\sj{$d \geq K$}\ba{I'm talking about semantic! why we need both d and k??} \sj{this is to be more general, the underlying feature space can have K dimensions that are semantically meaningful and the remaining $d-K$ dimensions can be noise. It's not an essential detail.}

The shared underlying feature helps us capture the notion that paired image-captions represent the same underlying object (feature) e.g. `\texttt{a dog}'. 
% Moreover, the unique feature for each latent class ensures that pairs in different latent classes do not represent the same underlying features. Note that for $i, j \in \Dpop^k$, while underlying features $\uf^i$ and $\uf^j$ both only have a non-zero element in the $k$-th coordinate, they are not equal. This represents the notion that while examples in the same latent class are similar, there is still significant variation amongst them e.g. an image-caption pair representing a golden retriever and a labrador are both in the dog latent class, and thus look similar but not equal as they capture the variation across these breeds of dogs.
The noise in the data distribution allows us to model both the occurrence of mismatched pairs e.g. an image of `\texttt{a dog}' matched with caption `\texttt{a cat}' as well as noise in data space for both images and texts e.g. an image of `\texttt{a dog with a cat in the background}' paired the caption `\texttt{a dog}' or the caption `\texttt{a dog with a cat}' paired with an image of `\texttt{a dog}'.

% Moreover, let $\mathcal{D}_V=\{(\xv^i, \xl^i)\}_{i\in V}$ be a set of $n=|V|$ image-caption pairs i.e. the full training data available to us, where $\xv^i$ denotes the image and $\xl^i$ denotes the caption of $i$-th example.

%Let $\mathcal{D}_V=\{(\xv^i, \xl^i)\}_{i\in V}$ be a set of $n=|V|$ image-caption pairs, where $\xv^i$ denotes the image and $\xl^i$ denotes the caption of $i$-th example. Moreover, let $\Dv = \{\xv^i \}_{i \in V}$ be the set of images and $\Dl = \{\xl^i \}_{i \in V}$ be the set of captions. Let the set of examples $V$ be partitioned into $K$ latent classes as follows: $V = \bigcup_{k \in [K]} V_k $. To model the notion that paired image-captions describe the same underlying object, let a given image-caption pair $(\xv^i, \xl^i)$ be generated as follows: $\xv^i = \Uv (\uf^i + \noisev)$ and $\xl^i = \Ul (\uf^i + \noisel)$ where: $\uf^i \in \mathbb{R}^d$ is the shared underlying feature vector of example $i$; $\Uv: \mathbb{R}^d \rightarrow \mathbb{R}^{\dv}$ and  $\Ul: \mathbb{R}^d \rightarrow \mathbb{R}^{\dl}$ are the mappings from underlying feature space to the vision and language data spaces, respectively; $\noisev, \noisel$ are the noise in underlying features for vision and language, respectively. For simplicity, we assume each latent class has a unique underlying feature, orthogonal to and sampled independently of the underlying features of other latent classes. Thus, equivalently, the $k$-th coordinate of the underlying feature vector corresponds to the underlying feature of latent class $k$. \footnote{This is equivalent to simply representing the underlying feature vector in the basis formed by the underlying features for each latent class}.  Finally, $\noisev, \noisel$ are sampled independently from each other and the underlying features; and $\norm{u} = \norm{\Uv} = \norm{\Ul} = 1$. 

%Let $\overline{\xv} = \Uv \uf$ be the noise-less equivalent of any image $\xv$ and similarly, $\overline{\xl} = \Ul \uf$ be the noise-less equivalent of any caption $\xl$. Moreover, $\overline{\D_V}$ be the noise-less equivalent of data $\D_V$. 

\textbf{Contrastive Language-Image Pre-training (CLIP)} CLIP is composed of a vision encoder $\fv: \mathbb{R}^{\dv} \rightarrow \mathbb{R}^K$ and a language encoder $\fl: \mathbb{R}^{\dl} \rightarrow \mathbb{R}^K$ that map input data in vision and language data space into a shared $K$-dimensional representation space, respectively (where $K$ is the number of latent classes as defined earlier). \ba{this is very confusing, I think this needs another projection matrix that maps any representation dimensionality to $K$, but here we say representation dimension is $K$ like it's a fact in CLIP! we should explain this.} 
The vision and language encoders are trained by maximizing the representation similarity of paired image-captions and minimizing that of unpaired image-captions in every mini-batch, using the following multimodal contrastive loss: \ba{note that we call $f$ and $F$ both encoders!! $f$ seems to be representations, fix this here and everywhere up to section 4.}\sj{f is the general function correpsonding to the vision and language encoders. In the special case of linear encoders, there is a matrix F which specifies the encoder. I'm not sure if I get what was wrong in the notation}
\begin{align}\label{eq:clip_loss}
    \!\!&\mathcal{L}_{\text{CLIP}}(\fv, \fl) \!=\! \nonumber \\
    -\!\!&\E_{\xv, \xl \sim \D} \!\log \frac{\exp({\fv(\xv)}^\top \fl(\xl))}{\E_{\xl^- \sim \mathcal{X}_{\mathcal{L}}} \exp({\fv(\xv)}^\top \fl(\xl^-))} \nonumber \\
   -\!\! &\E_{\xv, \xl \sim \D} \!\log \frac{\exp({\fv(\xv)}^\top \fl(\xl)}{\E_{\xv^- \sim \mathcal{X}_{\mathcal{V}}} \exp({\fv(\xv^-)}^\top \fl(\xl))}.
\end{align}
For simplicity of theoretical analysis, we consider linear encoders \ba{would be good to add a note about non-linear} where $\fv(\xv) = \Fv \cdot \xv$ and $\fl(\xl) = \Fl \cdot \xl$ where $\Fv \in \mathbb{R}^{r \times \dv}$ and $\Fl \in \mathbb{R}^{r \times \dl}$, \ba{$r$ or $K$?} used widely across machine learning literature \cite{pmlr-v206-nakada23a, ji2021power, pmlr-v202-xue23d}. Additionally, we use the linear multimodal contrastive loss used in \cite{pmlr-v206-nakada23a}:
\begin{align}\label{eq:lin_loss}
    \mathcal{L}(\Fv, \Fl)& = -\frac{1}{2n(n-1)}\sum_{i \in V}\sum_{\substack{j \in V \\ j\neq i}}(A_{ij} - A_{ii})\\ - 
    &\frac{1}{2n(n-1)} \sum_{i \in V}\sum_{\substack{j \in V \\ j\neq i}}(A_{ji}\!-\!A_{ii}) + \frac{\rho}{2}\| \Fv^\top \Fl \|_F^2, \nonumber
\end{align}
where $A_{ij}\coloneqq {(\Fv \xv^i)}^\top (\Fl \xl^j)$. \sj{\cite{pmlr-v206-nakada23a} shows that both the CLIP loss and the linear multimodal contrastive loss can be derived from the generalized multimodal contrastive loss that aligns representations of paired image-captions and separates representations of unpaired image-captions.} \ba{what's this?}

%Both the CLIP loss and the linear multimodal contrastive loss are derived from the same generalized  multimodal contrastive loss and achieve similar empirical performance \cite{pmlr-v206-nakada23a}.

Note that we only use linear encoders and the linear multi-modal contrastive loss function in our theoretical analysis; the experiments in Section \ref{sec:experiments} are conducted with non-linear encoders and the CLIP loss in Eq. \eqref{eq:clip_loss}.

\textbf{Zero-Shot Classification} After training, the model is evaluated via zero-shot classification on different downstream image classification tasks. A downstream task $\Dy$ is defined as a classification task on unseen data where the latent classes $\Dyy \subseteq [K]$ are a subset of latent classes of the pre-training data \ba{why subset?}. For zero-shot classification on downstream task $\Dy$, we use the language encoder $f_\mathcal{L}$ to encode the label %(e.g. the name of the class) corresponding to
of each latent class $y \in \Dyy$; then, the classification of an example $\xv$ is $zs_{f_V, f_L}(\xv) = \argmax_{k \in [K]} \frac{\fv{\xv} \cdot z_k}{\norm{\fv{\xv}}\norm{z_k}}$,
where $z_k = \E_{\xl s.t. y(\xl) = k}[\fl(\xl)]$ is the average representation of the label corresponding to class $k$ i.e. an example $\xv$ is classified by the closest (average) label representation. \sj{simplify to not talk about average} In practice, \cite{pmlr-v139-radford21a} proposed using a set of pre-engineered templates, e.g. `\texttt{A photo of a \{label\}}' to create several captions representing `\texttt{\{label\}}'. Thus, the average representation of the label would be the average of the representations of the templates obtained using $\fl$. The zero-shot error of $\fv, \fl$ is defined as the fraction of misclassified examples using the trained vision and language encoders $f_V, f_L$: \ba{fix this paragraph}
\begin{align}
\errzs{\fv, \fl} := \prob{\xv \sim \Dy}{y(\xv) \neq zs_{f_V, f_L}(\xv)}.
\end{align}
% \end{definition}


%For a given downstream classification task, let $\mathcal{Y} = \{y_i\}_{i=1}^r$ be the set of labels and $y(\xv)$ represent the label for example $\xv$. For both evaluations, we first obtain the image representations using the vision encoder $f_\mathcal{V}$. 

% \textbf{Linear Probe Error} For linear probe on downstream task $\Dy$, we train a linear classifier on the encoded representations such that the classification for an image $\xv$ is $g_{\fv, W}(\xv) := \argmax_k{({\fv(\xv)}^\top W)}_k$, where $W \in \mathbb{R}^{r \times |\Dyy|}$ is the weight of the trained linear classifier. The linear probing error of $f_V$ is defined as the error of the optimal linear classifier on the encoded representations of the downstream data:

% \begin{equation}
% \errlp{f_V} := \min_{W \in \mathbb{R}^{r \times |\Dyy|}} \prob{\xv}{y(\xv) \neq g_{\fv, W}(\xv)}.
% \end{equation}
% where $y(\xv)$ is the label for example $\xv$.

\textbf{Finding Generalizable Multimodal Subsets}

Our goal is to find a subset of training image-caption data $S \subseteq V$ of size at most $\ssize\geq|S|$, such that encoders trained on the subset achieve similar generalization, across downstream tasks using zero-shot evaluation, to encoders trained on the full training data $V$. To do so, we formulate the problem as finding a subset $S$ such that the encoders learnt on the subset closely approximate the encoders learnt on the full training data $V$:
\begin{align}\label{eq:problem_formulation}
   S^* = \argmins \norm{\Fvs - \Fv} + \norm{\Fls - \Fl}
\end{align}
where $\Fvs, \Fls$ are the vision and language encoders learnt on the subset $S$ and $\Fv, \Fl$ are the encoders learnt on the the full training data $V$. 
%\sj{better now?: \ap{ Why is defining the goal as such meaningful ?. Does this guarantee the zeroshot/linearProbe classification performance? If we are showing this later, maybe we need to just point this out.}}

%\sj{Improve: With the encoders learnt on the subset $S_*$ closely approximating the encoders learnt on the full data $V$, the generalization performance on downstream tasks using these encoders will be similar. Thus, performance across 1) linear probe evaluation: performance on an image-classification task of a linear classifier trained on the representations of images obtained from the vision encoder;  and 2) zero-shot classification - classification based on similarity of the text representations of the labels and the image encoders images.}

%\sj{change to feature version, but motivate noiseless from here?}
%\textbf{Finding Generalizable Multimodal
%Subsets} Our goal is to find a subset $S\subseteq V$ with size at most $n_S \leq n$ that achieves a similar or superior zero-shot and linear probe error compared to that of the encoders trained on the full data. Formally,

%\begin{align}\label{eq:problem_formulation} S^* = \argmin_{S\subseteq V, |S|\leq n_s} \delta_{lp} + \delta_{zs},
%\end{align}

%where $\delta_{lp}=|\errlp{f_V}-\errlp{f_V^S}|$ and $\delta_{zs}=|\errzs{f_V, f_L}-\errzs{f_V^S, f_L^S}|$.

%\textbf{Practical Considerations}

%\sj{In practice, the pre-training data is not the population but rather sampled from it, and as a result is likely to be 1) imbalanced 2) ce}. We address this in 





==> tables/main_results.tex <==
\begin{table}[htbp]\label{table:subset_sizes}
\caption{Comparing performance of Baselines and \method across Tasks for different subset sizes}
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|}
Subset Size               & Method                          & ImageNet ZS      & Shifted ImageNet ZS & Average LP       & Average ZS       \\
\hline \hline \\
\multirow{6}{*}{10\%}     & Random                          & 4.00\%           & 2.44\%                  & 43.21\%          & 10.43\%          \\
                          &CLIP Score (Lowest)                            & 0.57\%           & 0.60\%                  & 34.29\%          & 6.41\%           \\
                          & CLIP Score                           & 6.35\%           & 4.46\%                  & 49.94\%          & 11.84\%          \\
                          & SemDeDup                        & 2.13\%           & 1.62\%                  & 39.80\%          & 9.29\%           \\
                          & C-RHO                          & 0.91\%           & 1.01\%                  & 35.16\%          & 6.84\%           \\
                          & \textbf{\method} & \textbf{11.33\%} & \textbf{5.97\%}         & \textbf{53.13\%} & \textbf{14.72\%} \\
\hline \\                          
\multirow{6}{*}{20\%}     & Random                          & 6.70\%           & 3.89\%                  & 45.05\%          & 13.62\%          \\
                          &  CLIP Score (Lowest)                            & 1.38\%           & 0.97\%                  & 33.01\%          & 7.06\%           \\
                          & CLIP Score                           & 11.38\%          & 6.73\%                  & 52.55\%          & 17.93\%          \\
                          & SemDeDup                       & 4.83\%           & 2.83\%                  & 40.40\%          & 11.23\%          \\
                          & C-RHO                         & 4.10\%           & 2.73\%                  & 39.60\%          & 11.04\%          \\
                          & \textbf{\method} & \textbf{15.86\%} & \textbf{9.24\%}         & \textbf{57.32\%} & \textbf{20.59\%} \\
\hline \\                            
\multirow{6}{*}{30\%}     & Random                          & 9.77\%           & 5.33\%                  & 48.01\%          & 16.40\%          \\
                          & CLIP Score (Lowest)                            & 2.64\%           & 1.61\%                  & 35.80\%          & 9.86\%           \\
                          & CLIP Score                         & 14.77\%          & 8.53\%                  & 54.99\%          & 20.97\%          \\
                          & SemDeDup                       & 8.36\%           & 4.55\%                  & 45.60\%          & 14.48\%          \\
                          & C-RHO                           & 9.14\%           & 5.59\%                  & 46.88\%          & 15.48\%          \\
                          & \textbf{\method} & \textbf{17.91\%} & \textbf{10.59\%}        & \textbf{58.51\%} & \textbf{22.87\%} \\
\hline \\  
\multirow{6}{*}{40\%}     & Random                          & 11.91\%          & 6.65\%                  & 50.60\%          & 18.33\%          \\
                          &  CLIP Score (Lowest)                            & 4.66\%           & 2.52\%                  & 41.97\%          & 11.65\%          \\
                          & CLIP Score                            & 17.04\%          & 10.01\%                 & 57.70\%          & 23.67\%          \\
                          & SemDeDup                        & 10.99\%          & 6.11\%                  & 48.67\%          & 18.00\%          \\
                          & C-RHO   & 12.25\%          & 7.31\%                  & 50.54\%          & 19.85\%          \\
                          & \textbf{\method} & \textbf{RUNNING} & \textbf{RUNNING}        & \textbf{RUNNING} & \textbf{RUNNING} \\
\hline \\                            
\multirow{6}{*}{50\%}     & Random                          & 13.37\%          & 7.50\%                  & 52.69\%          & 20.76\%          \\
                          &  CLIP Score (Lowest)                            & 6.54\%           & 3.52\%                  & 44.75\%          & 14.00\%          \\
                          & CLIP Score                         & 18.68\%          & 11.02\%                 & 58.92\%          & 24.59\%          \\
                          & SemDeDup                        & 13.30\%          & 7.57\%                  & 51.47\%          & 21.11\%          \\
                          & C-RHO                           & 14.94\%          & 8.65\%                  & 53.11\%          & 21.23\%          \\
                          & \textbf{\method} & \textbf{RUNNING} & \textbf{RUNNING}        & \textbf{RUNNING} & \textbf{RUNNING} \\
\hline \\                            
100\% & Full Data                       & 19.53\%          & 11.58\%                 & 58.87\%          & 26.24\%  
\end{tabular}
\end{small}
\end{table}
